Parameterized Model Checking of Token-Passing Systems

We revisit the parameterized model checking problem for token-passing systems and specifications in indexed $\textsf{CTL}^\ast \backslash \textsf{X}$. Emerson and Namjoshi (1995, 2003) have shown that parameterized model checking of indexed $\textsf{CTL}^\ast \backslash \textsf{X}$ in uni-directional token rings can be reduced to checking rings up to some \emph{cutoff} size. Clarke et al. (2004) have shown a similar result for general topologies and indexed $\textsf{LTL} \backslash \textsf{X}$, provided processes cannot choose the directions for sending or receiving the token. We unify and substantially extend these results by systematically exploring fragments of indexed $\textsf{CTL}^\ast \backslash \textsf{X}$ with respect to general topologies. For each fragment we establish whether a cutoff exists, and for some concrete topologies, such as rings, cliques and stars, we infer small cutoffs. Finally, we show that the problem becomes undecidable, and thus no cutoffs exist, if processes are allowed to choose the directions in which they send or from which they receive the token.

==> CompositionProof.tex <==
\section{Proof of Reduction + Finiteness Theorems}

\subsection{Discussion of method for proving cutoffs} \label{discussion:method}

Before introducing the relevant definitions we discuss the key ideas behind the method.
\todo{Method..: a citation of `the composition method' paper}

\todo{Give purpose of $P^G|\bar{g}$ and $G|\bar{g}$. Add intuition.}

\todo{Say how the method extends or differs from known methods}

\paragraph{Discussion.}
\todo{Integrate this discussion into the next sections or move to appendix to save space}
Fix a non-indexed temporal logic \TL, such as \dCTLstarmX.
In a $k$-indexed \TL\ formula $(Q_1 x_1) \cdots (Q_k x_k)\ \varphi$ every assignment $e$ of the variables $x_1, \cdots, x_k$ designates $k$ nodes of the underlying topology $G$, with the semantic that an atomic proposition $p_x$ 
 is interpreted by looking at the state of the process at $e(x)$. The assignment $e$ is represented as the $k$-tuple $\bar{g} = (g_1,\cdots,g_k)$. The formula $\varphi$ can only talk about $\bar{g}$.
 
In order to prove that PMCP has a cutoff it is natural to find conditions on two topologies $G,G'$ and $\bar{g},\bar{g}'$ that allow one to conclude that $P^G$ and $P^{G'}$ are indistinguishable with repect to $\varphi$. 

Ignoring initial states for now, we define $\tokengraphnoinit{G}{\bar{g}}$ to be the LTSs such that each state $g_i$ has an atom that identifies it, while no atoms hold at any state not in $\bar{g}$ (Section~\ref{sec:method}).

Similarly we define $\abstractionnoinit{P^G}{\bar{g}}$ to be the LTSs like $P^G$ except that the labeling of a global state $s$ ensures that an atom indexed by $v \in \bar{g}$ carries the position of $v$ in $\bar{g}$. Atoms indexed by $v \not\in \bar{g}$ are removed (Section~\ref{sec:method}). \note{add initial state} Thus `$P^G$ and $P^{G'}$ are indistinguishable with respect to $\varphi$' can be formalised as `$P^G|\bar{g}$ is indistinguishable from $P^{G'}|\bar{g}$'.

So, when is $\abstractionnoinit{P^G}{\bar{g}}$ indistinguishable from $\abstractionnoinit{P^{G'}}{\bar{g}'}$? Intuitively, this will happen if the states of the processes at the nodes of $\bar{g}$ in $P^G$ and the corresponding nodes of $\bar{g}'$ in $P^{G'}$ are always able to change in exactly the same ways, as far as $\varphi$ can detect. Recall from the definition of token-passing system (in Section~\ref{dfn:paramsys}) that a state of a process at a node $g$ of $G$ can change in exactly two ways:
\begin{enumerate}
\item the process at $g$ takes a local transition of $P$ that does not involve any
token movement, or
\item the process at $g$ sends or receives the token.
\end{enumerate}

Changes of the form (1) can easily be mimicked by the process at a node $g'$ of $G'$,
regardless of the strucure of the graph $G'$; whereas whether or not
changes of the form (2) can be mimicked in $P^{G'}|\bar{g}'$ depends on the structure of
$P^{G'}|\bar{g}'$. A key observation is that for processes that are not direction-aware, i.e., $P \in \Psimptok$, or for topologies in which direction sensing is not relevant, such as uni-directional rings,  the ability
of $P^{G'}|\bar{g}'$ to mimick the token movements in
$P^G|\bar{g}$  (and vice versa) does not depend on the process $P$, but only on the structure
of the graphs $G$ and $G'$. This observation is
at the heart of why the $\Psimptok$ case is decidable, while the other cases $\Psnd$, $\Prcv$, and $\Prcvsnd$ are not.

\sr{Add comment that the $k$-topology of CTTV  satisfies the assumption of the reduction ppt}

%Below, we formally substantiate this observation
%and provide a condition on $G$ and $G'$ that completely characterizes when $P^G,g-bar$
%and $P^{G'}-g'-bar$ are indistinguishable with respect to suffixes $\phi$ of
%formulas in $TL$ (with respect to the given assignments $g-bar, g'-bar$). In order to capture
%the possible ways the token can move in $G$ between the nodes identified by the
%assignment $g-bar$ (similarly for $G'$ and $g'-bar$) we consider the TLS
%$(G,token(s),g-bar$ ($(G',token(s'),g'-bar$) which is simply
%the graph $G$ ($G'$) where for every $i \in [k]$ the node assigned by $g-bar$ ($g'-bar$) to
%the $i$'th variable is labeled by an atomic proposition $i$.
%Observe that a suffix of a formula in $TL$ with (with atomic propositions $1..k$) interpreted
%over $(G,token(s),g-bar$ ($(G',token(s'),g'-bar)$) is actually
%a specification of possible ways a token can move in $G$ $(G'$). 
The \textsc{reduction} property states that the intuitive
notion of whether $P^G_s|\bar{g}$ and $P^{G'}_{s'}|\bar{g}'$ are able to mimick each other's
possible token movements (as far as the nodes designated by $\bar{g}$ and $\bar{g}'$ are concerned, and starting in states $s$ and $s'$) is exactly captured by the $TL$ equivalence of $\tokengraph{G}{\token(s)}{\bar{g}}$ and
$\tokengraph{G'}{\token(s')}{\bar{g'}}$. 

To get a cutoff it is now enough to establish a \textsc{finiteness} property that states that there are finitely many topologies of the form $\tokengraph{G}{\token(s)}{\bar{g}}$ up to $\TL$-equivalence. 

There are many standard finiteness lemmas: for instance for every integer $b$ there are finitely many formulas, up to equivalence, from the set of \LTLmX\ formulas that have nesting depth of temporal operators at most $b$.

In Section~\ref{section:finiteness} we will prove that (arbitrary) $\pgraph$ has the finiteness property with respect to the logic \dCTLstarmX. In particular this holds for $d = 1$ and thus for \LTLmX.

\sj{why is the following part important?}\sr{It is important because it shows that the finiteness property is not trivial/automatic (as I thought it would be originally). However, this sort of note can go before the proof, in the appendix.} Note that the finiteness property is false if instead of using graphs of the form $(G,x)|\bar{g}$ we use arbitrary LTSs. Indeed, there are infinitely many \LTLmX\ formulas that are pairwise logically-inequivalent. E.g., let $M$ be a chain over atom $\{a\}$; thus we may think that $M$ represents a finite word over binary alphabet $\{0,1\}$. Then \LTL\ formulas, using next, can spell out any word. A slight variation using 'until' also works for \LTLmX. 
Thus the proof of the finiteness property for \dCTLstarmX\ must, and does, exploit the structure of the LTS $(G,x)|{\bar{g}}$. \todo{finish discussion of finiteness ppt}


\subsection{Reduction Theorem} \label{section:reduction}

\begin{reptheorem}{theorem:reduction}[\textbf{Reduction}]
For all integers $d,k$, graphs $G,G'$, process $P \in \Psimptok$, global states $s$ of $P^{G}$ and $s'$ of $P^{G'}$,
 %such that $s(x)$ has the token and $t(y)$ has the token, 
 $k$-tuple of distinct elements ${\bar{g}}$ over $V_G$ and  $k$-tuple of distinct elements ${\bar{g}'}$ over $V_{G'}$:
 \begin{quotation}
If $s(g_i) = s'(g'_i)$ for $1 \leq i \leq k$ and 
$\tokengraph{G}{\token(s)}{\bar{g}} \equiv_{\dCTLstarmX}  \tokengraph{G'}{\token(s')}{\bar{g}'}$
%where $\token(s) = x$ and $\token(s') = x'$, 
then 
%(g_i) = t(h_i)$ for $1 \leq i \leq k$ and $(G,x)|{\bar{g}} \equiv_{\dCTLstarmX} (H,y)|{\bar{h}}$ then 
$\abstraction{P^{G}}{s}{\bar{g}} \equiv_{\dCTLstarmX} \abstraction{P^{G'}}{s'}{\bar{g}'}$.
\end{quotation}
\end{reptheorem}

Before proving the Theorem we state some lemmas which follow from property vii) in the definition of process template and the fact that the internal state of a process with (without) the token does not determine to (from) which node the token is sent (received), i.e., processes are not direction-aware.

\begin{lemma}[Fairness] \label{lem:fairness}
Fix finite $P \in \Psimptok$ and system $P^G$. In every infinite path $\pi$ of $P^G$ there are infinitely many token-passing transitions.
\end{lemma}

\begin{lemma}[Priming to send/receive] \label{lem:priming}
Fix $P \in \Psimptok$, system $P^G$, global state $s_1$, and some $x \in V_G$. Then there is a path $s_1 \cdots s_t$ (for some $t$) in $P^G$ such that i) for all $y \neq x$ and $1 \leq j \leq t$, we have $s_j(y) = s_1(y)$, and ii) if $\token(s_1) = x$ then $s_t(x)$ is send-only, and iii) if $\token(s_1) \neq x$ then $s_t(x)$ is receive-only.\sj{mention that given $P$, there is a fixed upper bound on $t$?\\(SR) not needed.} Moreover the path $s_1 \cdots s_t$ does not contain a transition with action $\tsnd$ or $\trcv$.
\end{lemma}


\begin{lemma}[Token pushing] \label{lem:tokenpushing}
\sj{This lemma is hard to grasp. We should give some informal idea first. Even I currently don't see why it contains $\bar{g}$. \\
To make it easier to read, we could replace $s$ with $s_1$, $f_0 \ldots f_t$ with $s_1 \ldots s_t$, and remove ``starting in $s$''. Then, in 2., 0 changes to 1, and in 3., 1 to 2.}
Fix $P \in \Psimptok$, let $p,q$ be states of $P$, and let $G$ be a topology, and a $k$-tuple $\bar{g}$ over $V_G$. Let $x_1 x_2 \cdots x_n$ be a simple path in $G$ and let $s$ be a global state of $P^G$ such that i) $\token(s) = x_1$, ii) there is a transition $\trans{s(x_1)}{p}{\tsnd}$ in $P$, iii)  there is a transition $\trans{s(x_n)}{q}{\trcv}$ in $P$, iv) for all $y \not\in\{ x_1,x_n\} \cup \{g_1, \cdots, g_k\}$, we have $s(y)$ is receive-only.

 Then there exists a path $f_0 \cdots f_t$ (for some $t$) in $P^G$ starting in $s$ such that 
\begin{enumerate}
\item removing successive identical elements from the sequence $\token(f_0) \cdots \token(f_t)$ yields the path $x_1 \cdots x_n$,
\item if $0 \leq j \leq t$ and $x$ not on the path $x_1 \cdots x_n$ then $f_j(x) = s(x)$.
\item $f_j(x_1) = p$ for $1 \leq j \leq t$;
\item $f_j(x_n) = f_0(x_n)$ for $1 \leq j < t$, and $f_t(x_n) = q$.


\end{enumerate}
\end{lemma}



\subsubsection{Proof of Theorem \ref{theorem:reduction}(Reduction).}


\begin{proof}\note{Clean up proof: 1. define $block_\pi(n)$ gives the block}
%Here is an outline of the structure of the proof. We transfer a winning strategy in the $d$-round game between $G,H$ to one between $P^G$ and $P^H$. If Spoiler picks a path in $P^G$ then project this to a path in $G$ which records where the token is (we may assume that the projection does not stutter, except possibly in an infinite tail). Use the winning strategy between $G,H$ to find a path in $H$ and pull this up to $P^H$ by  moving the token as in $H$ and scheduling the other $k$ important processes as in the path in $P^G$. The paths in $P^H,P^G$ are stuttering equivalent and so Duplicator can survive the round.
\todo{check notation, in proof, of $\abstraction{P^G}{s}{\bar{g}}$ and $\tokengraph{G}{x}{\bar{g}}$}


Fix $k,s,s',G,G',P,\bar{g},\bar{g}'$.\ak{what is the scope of this 'fix'? the whole proof or just for the property?} We induct on $d$. The induction hypothesis states: 
 \begin{quotation}
For every\ak{no need of `for every t/t' ' -- use s,s'?} $t$ in $P^G$ and $t' \in P^{G'}$, if $t(g_i) = t'(g'_i)$ for $i \leq k$ and $\token(t) \equiv_d \token(t')$, then 
$t \equiv_d t'$.
\end{quotation}

Note that the equivalence $\equiv_d$ in the expression $\token(t) \equiv_d \token(t')$ is with respect to LTSs 
$\tokengraph{G}{\token(s)}{\bar{g}}$ and $ \tokengraph{G'}{\token(s')}{\bar{g}'}$; and the equivalence $\equiv_d$ in the expression $t \equiv_d t'$ is with respect to LTSs $\abstraction{P^{G}}{s}{\bar{g}}$ (with labeling function $L$) and $\abstraction{P^{G'}}{{s'}}{{\bar{g}'}}$ (with labeling function $L'$).\sj{I don't understand where this relation comes from (or why it is renamed here, if it is the same as the previously defined one(s)).}

By Proposition~\ref{prop:equiv} the induction hypothesis for $d$ implies that the theorem holds for $d$.


\paragraph{Base case.}
For the base case let  $d = 0$ and take $t,t'$. Then $t(g_i) = t'(g'_i)$ for $i \leq k$ implies that $t$ and $t'$ have the same label since 
 $p@i \in L(t)$ iff $p_{g_i} \in \Lambda(t)$ iff $p \in \lambda(t(g_i))$ iff $p \in \lambda(t'(g'_i))$   iff $p_{g'_i} \in \Lambda'(t')$ iff $p@i \in L'(t')$.\note{make readable} Thus by definition of $\equiv_0$ we have $t \equiv_0 t'$, so the base of the induction holds.
  

\paragraph{Inductive step.}
Suppose $d > 0$ and the induction hypothesis holds for all $l < d$. We show it holds for $d$. To that end take $t,t'$ and assume $(\ast)$:
$t(g_i) = t'(g'_i)$ for $i \leq k$ and  $x \equiv_d x'$ where $x := \token(t)$ and $x' := \token(t')$. We show that $t \equiv_d t'$.

Let $\pi = \pi_1 \pi_2 \cdots$ be an infinite path in $\abstraction{P^G}{t}{\bar{g}}$. We form a path $\rho$ of $\tokengraph{G}{\token(s)}{\bar{g}}$ starting in $x$ that records the token movement along $\pi$,  by deleting consecutive identical elements in the sequence $\token(\pi_1) \token(\pi_2) \cdots$. Formally, define $proj_\pi:\Nat \to \Nat$ as follows: $proj_\pi(0) := 0$ and otherwise $proj_\pi(i) := proj_\pi(i-1)$ if $\token(\pi_{i-1}) = \token(\pi_i)$ and $proj_\pi(i) := proj_\pi(i-1) + 1$. Define $\rho_i := \token(\pi_j)$ where $j$ is the least integer such that $proj_\pi(j) = i$. Note that by Lemma~\ref{lem:fairness} $\rho$ is an infinite path. Note that if $i < j$ then $proj_\pi(i) \leq proj_\pi(j)$.

\paragraph{Definition of $\rho'$.} Since $x \equiv_d x'$ there exists an infinite path $\rho'$ of $\tokengraph{G'}{\token(s')}{\bar{g}'}$ starting in $x'$, and partitions $B_1B_2\cdots$ of $\rho$ and $B'_1B'_2\cdots$ of $\rho'$, such that for each $i$ and $b \in B_i, b' \in B'_i$ it holds that $\rho_b \equiv_{d-1} \rho'_{b'}$. 

Note $1$. Without loss of generality we assume that for every $m$, if $i,j \in B'_m$ then $\rho'_i \neq \rho'_j$ (one can simply remove cycles within a block). 

Note $2$: Suppose $\rho_i  = g_j$ for some $j$. Then $\rho_i$ is labeled $\{j\}$ and is the only node of $G$ with this label. Recall from the note after Definition~\ref{dfn:equiv} that nodes of $\rho$ whose positions are in the same block must agree on their labels. Conclude that the $B$-block containing $i$ is exactly $\{i\}$. Similarly if $\rho'_i  = g_j$ for some $j$ then the $B'$-block containing $i$ is exactly $\{i\}$\ak{typos? should be $\{\rho_i\}$?}. 


\

In the remainder of the proof we show there exists an inifinite path $\pi'$ of $\tokengraph{P^{G'}}{s'}{\bar{g}'}$ starting in $t'$ 
%such that $\rho'$ records the token movement along $\pi'$, 
and partitions $A_1A_2\cdots$ of $\pi$ and $A'_1A'_2\cdots$ of $\pi'$ such that for each $i$ and $a \in A_i, a' \in A'_i$\ak{typos? should be $\pi_a$?} it holds that $\pi_a \equiv_{d-1} \pi'_{a'}$. Thus by definition~\ref{dfn:equiv} we have that $t \equiv_d t'$ holds, and this would complete the proof of the inductive step, and thus the theorem.


 
We construct $\pi'$ step by step as follows. Throughout the construction we maintain integers $l,l'$ satisfying the following invariants $(\dagger)$: 
\begin{itemize}
\item[i.] the first $l$ elements of $\pi$ have been considered and assigned to blocks $A_1,A_2,\cdots, A_n$ (for some $n$);
\item[ii.] the first $l'$ elements of $\pi'$ have been defined and have been assigned to blocks $A'_1,\cdots, A'_n$;
\item[iii.] for every $j \leq n$ and $a \in A_j, a' \in A'_j$ we have $\pi_a(g_i) = \pi'_{a'}(g'_i)$ for $i \leq k$;

\item[iv.] for all $j \leq n$ there exists integer $m$ such that for every $a \in A_j, a' \in A'_j$ we have $proj_\pi(a)$ is in block $B_m$ and $proj_{\pi'}(a')$ is in block $B'_m$.
\end{itemize}

Note that by the third and fourth invariants, for every $j \leq n$, and $a \in A_j, a' \in A'_j$, 
the left-side of the implication in the $d-1$ inductive hypothesis holds for 
 $t = \pi_a$ and $t' = \pi'_{a'}$. Thus $\pi_a \equiv_{d-1} \pi'_{a'}$.
 
\paragraph{Construction.}
We now describe the construction of $\pi'$ and the partitions $A_1, A_2, \cdots$ and $A'_1,A'_2, \cdots$. 

It is initialized with $l = l' = 1$ and $A_1 = A'_1 = \{1\}$. Each step of the construction proceeds in two phases.

In the first phase: iterate Lemma~\ref{lem:priming} for $y \not \in \bar{g}'$ to obtain a path $f_0 \cdots f_h$ such that $f_1 = \pi'_{l'}$ and $f_h(y)$ for $y \not \in \bar{g}'$ is either send-only or receive-only. Append $f_1 \cdots f_h$ to $\pi'$, add $l'+1, \cdots, l'+h$ to $A'_n$.

In the second phase consider the transition from $\pi_l$ to $\pi_{l+1}$. There are three cases.
 
 \begin{enumerate}
 \item If it is an internal transition of a process not in $\bar{g}$ then extend block $A_n$ to include $l+1$. In this case $l'$ does not change.
 \item  If it is an internal transition of a process in some $g_i$ from $\bar{g}$, say from local state $q$ to $q'$, then i) put $l+1$ in a new block $A_{n+1}$, ii) define $\pi'_{l'+1}$ to be the global state resulting from $\pi'_{l'}$ by changing the local state of the process $g'_i$ from $q$ to $q'$, iii) put $l'+1$ in a new block $A'_{n+1}$. 
 \item If it is a token-passing transition, i.e., $\token(\pi_l) \neq \token(\pi_{l+1})$, then there are two subcases:
 \begin{enumerate}
 
 \item if $proj_\pi(l)$ and $proj_\pi(l+1)$ are in the same $B$-block then extend block $A_n$ to include $l+1$. In this case $l'$ does not change.
 
 \item if $proj_\pi(l)$ and $proj_\pi(l+1)$ are in different (and hence successive) $B$-blocks, say $B_m$ and $B_{m+1}$, then put $l+1$ in a new block $A_{n+1}$. Let $y = proj_{\pi'}(l')$ and note that by the third invariant $y$ is in block $B'_m$ and let $z$ be the first position in block $B'_{m+1}$. 



 
% If $\token(\pi_l) \in \bar{g}$ let $p = \pi_{l+1}(\token(\pi_l))$ otherwise

 To apply  Lemma~\ref{lem:tokenpushing} we let $p = \pi_{l+1}(\token(\pi_l))$ if $\token(\pi_l) \in \bar{g}$, and otherwise let $p$ be any local state such that there is a transition $\trans{\pi'_{l'}(\rho'_y)}{p}{\tsnd}$ in $P$.
 Similarly let $q = \pi_{l+1}(\token(\pi_{l+1}))$ if $\token(\pi_{l+1}) \in \bar{g}$, and otherwise let $q$ be any local state such that there is a transition $\trans{\pi'_{l'}(\rho'_z)}{q}{\trcv}$ in $P$.

Now apply the Lemma~\ref{lem:tokenpushing} with path $\rho'_y \rho'_{y+1} \cdots \rho'_{z}$ and global state $\pi'_{l'}$ and local states $p,q$ to get a finite path $f = f_0 \cdots f_t$ (for some $t$) in $\abstraction{P^{G'}}{s'}{\bar{g}'}$ starting in $\pi'_{l'}$.\sr{the initial state $s'$ is no longer used. there should be better notation}


Extend the path $\pi'$ by appending $f_1 \cdots f_t$ to it (so $l'$ increases by $t$). 
 
 
 Extend block $A'_{n}$ to include $(l'+1), \cdots, (l'+t-1)$. Put $l'+t$ into a new block $A'_{n+1}$. 
 

% Add $l'+1 there is a finite path $f$ from $\rho'(i')$ to  in $\pi'[l]$ that results in the token moving from the process with index $\rho'[proj_\pi'(l)]$ to the last process in block $B'_n$, append $f$ to the $A'_n$-block, iii) letting $e$ be a finite path starting in the last state of $f$ that results in the token moving to the next process index in $\rho'$, append $e$ to $\pi'[l']$ and put these in a new block $A'_{n+1}$.\note{rough}
 \end{enumerate}
\end{enumerate}
 
\paragraph{The construction is well-defined.}

\begin{itemize}
\item The construction gives an infinite path $\pi'$. Indeed, since $l$ increases at each step, then by Lemma~\ref{lem:fairness} infinitely often the construction is in case 3, and since the $B$-blocks are finite, infinitely often the construction is in case 3b), so infinitely often $\pi'$ is extended.
\item In case 3(b) we need to show that Lemma~\ref{lem:tokenpushing} is correctly applied. By Note $1$. the path $\rho'_{y} \rho'_{y+1} \cdots \rho'_{z}$ is a simple path. 
The first phase of the step ensures that every $w \not\in \bar{g}'$ is send-only or receive-only, thus together with the third invariant, our choice of $p$ and $q$ ensures that the lemma is applicable.
\end{itemize}



 \paragraph{The construction maintains the invariants $(\dagger)$.}
 
At the beginning of the construction the third invariant follows from the assumption $(*)$ and the other three invariants are immediate.

Suppose at the start of a step the maintained integers are $l,l'$ and the invariants $(\dagger)$ hold. We argue that the invariants hold after the step.

The invariants hold after the first phase: the first two invariants are immediate. For the third note that $\pi_l(g_i) = \pi_{l'}(g'_i) = \pi'_{l'+1}(g'_i) = \cdots = \pi'_{l'+t}(g'_i)$ by Lemma~\ref{lem:priming}. The fourth invariant holds because $proj_{\pi'}(l') = proj_{\pi'}(l'+1) = \cdots = proj_{\pi'}(l'+t)$ since the token did not move in this phase.

We now assume that $(\dagger)$ holds for $l,l'$ at the end of the first phase, and show the invariants hold at the end of the second phase. It is immediate from the construction that the first two invariants are maintained. 

\paragraph{Invariant three, phase two.} For the third invariant we consider each case separately. In case 1) we have to show that for $j \leq k$, $\pi_{l+1}(g_i) = \pi_l(g_i)$. But this follows since $\pi_{l+1}(g_j) = \pi_l(g_j)$ (because the transition from $\pi_l$ to $\pi_{l+1}$ did not change the state of the process $g_j$) and $\pi_l(g_j) = \pi_{l'}(g_j)$ (because the third invariant held at the beginning of the step).

In case 2) we have to show that for $j \leq k$, $\pi_{l+1}(g_j) = \pi_{l'+1}(g_j)$. This is immediate from the construction since for $j \neq i$ we have $\pi_l(g_j) = \pi_{l+1}(g_j)$, and $\pi_{l+1}(g_i) = q' = \pi_{l'+1}(g_i)$.

In case 3(a) the token moved but the $B$-block did not change. Thus by Note $2$ the token-passing transition did not involve any of the processes in $\bar{g}$. Now use the same argument as in case 1).

In case 3(b) it is enough to show that for $1 \leq i \leq k$ it holds that $\pi_{l+1}(g_i) = f_t(g'_i)$ and for every $1 \leq j \leq t-1$ it holds that $\pi_l(g_i) = f_j(g'_i)$. Fix $i$.   Observe that $g'_i$ can not appear on the path $\rho'_{y} \rho'_{y+1} \cdots \rho'_{z}$ except as the first or last nodes of the path (since by construction ${y+1}, \cdots, {z-1}$ are all in the same $B'$-block as $y$, thus by Note $2$. the nodes $\rho'_{y+1}, \cdots, \rho'_{z-1}$ are not in $\bar{g}'$).  Also observe that by our choice of $y,z$ we have that $\rho'_y \equiv_{d-1} \token(\pi_l)$ and $\rho'_z \equiv_{d-1} \token(\pi_{l+1})$. 

There are three subcases to consider.  First subcase: $g_i \neq \token(\pi_l)$ and $g_i \neq \token(\pi_{l+1})$. In particular $\rho'_y \neq g'_i$ and $\rho'_z \neq g'_i$ (since $\equiv_{d-1}$ implies $\equiv_0$, and $g'_i$ is $\equiv_0$ only to $g_i$). Thus $g'_i$ does not appear on the path $\rho'_{y} \cdots \rho'_{z}$. Then
 for $1 \leq j \leq t$ we have  $f_j(g'_i) = \pi_{l'}(g'_i) = \pi_l(g_i)   = \pi_{l+1}(g_i)$ (the first equality is by Lemma~\ref{lem:tokenpushing}, the second by the third invariant, the third since $g_i \neq \token(\pi_l), \token(\pi_{l+1})$ implies that $g_i$ is not involved in the token-passing transition from $\pi_l$ to $\pi_{l+1}$).
 
Second subcase: $g_i = \token(\pi_{l+1})$. Then for $1 \leq j < t$, we have $f_j(g'_i) = \pi'_{l'}(g'_i) = \pi_l(g_i)$. The first equality holds by item 4. of Lemma~\ref{lem:tokenpushing}, and the second by the third invariant assumption at the beginning of the phase. By construction and item 4. of the lemma, we have $f_t(g'_i) = q = \pi_{l+1}(g_i)$.

Third subcase: $g_i = \token(\pi_l)$. Thus by the second observation above $g_i \equiv_{d-1} \rho'_y$. But this means that $\rho'_y = g'_i$. Now, $\pi_{l+1}(g_i) = p = f_t(g'_i)$ by construction. We claim that $t = 1$ and so $\pi_l(g_i) = f_j(g'_i)$ ($1 \leq j \leq t-1$) holds vacuously. Indeed: by Note $2$. and our choice of $y,z$, the fact that $g'_i = \rho'_y$, we have $z = y+1$. Observe that $\token(f_0) \neq \token(f_1)$ because by item 3. of Lemma~\ref{lem:tokenpushing} the transition from $f_0$ to $f_1$ is a token-passing transition. By item 1. of the lemma $\token(f_1)$ must equal $\rho'_z$.
By item 4. of the lemma the token arrives at $\rho'_z$ only by the transition from $f_{t-1}$ to $f_t$. Thus $t = 1$ as promised.

 
\


\paragraph{Invariant four, phase two.}
We check the fourth  invariant for each case separately.
In case 1) the fourth invariant holds because $proj_{\pi}(l) = proj_{\pi}(l+1)$ since the token did not move.

In case 2) the fourth invariant holds because  $proj_{\pi}(l) = proj_{\pi}(l+1)$ and $proj_{\pi'}(l') = proj_{\pi'}(l'+1)$ since in both transitions the token did not move.

Case 3a) is immediate.

For case 3b) consider the nodes $f_1 \cdots f_{t-1}$ whose positions were added to the block $A'_n$. By item 1. of Lemma~\ref{lem:tokenpushing} $\{\token(f_0), \cdots,\token(f_{t})\} = \{\rho'_y, \cdots, \rho'_z\}$. Then by item 4. of the lemma we  get  $\{\token(f_0), \cdots,\token(f_{t-1})\} = \{\rho'_y, \cdots, \rho'_{z-1}\}$ since the token arrived at $\rho'_z$ only at the transition from $f_{t-1}$ to $f_t$. 
Hence $\{proj_{\pi'}(l'), \cdots, proj_{\pi'}(l'+t-1)\} = \{y, y+1, \cdots, z-1\}$.

By construction $y, \cdots, {z-1}$ are in $B'_m$. In other words, the new nodes $\pi'_{l'+1}, \cdots, \pi'_{l'+t-1}$ are in the same $A'$-block as $\pi'_{l'}$ and their projections are in the same $B'$-block as $proj_{\pi'}(l')$, as required.

Finally, we show that $l+1 \in A_{n+1}$ and $l'+t \in A'_{n+1}$ project to blocks with the same index. Indeed: by assumption we have that $proj_{\pi}(l+1) \in B_{m+1}$, and by our choice of $z$ we have $z \in B'_{m+1}$. Observe that 
$proj_{\pi'}(l'+t) = z$ since $\rho'_y, \cdots, \rho'_z$ is a simple path and $\token(\pi'_{l'+t}) = \rho'_z$. This completes the proof.
\qed
\end{proof}

% casewe proceedfollows from the fact that only place in the construction where $proj_\pi(l)$ or $proj_{\pi'}(l')$ change is in step 3). Indeed, suppose before step 3a) the integers maintained are $l,l'$, so after the step they are $l+1,l'$. Since $proj_\pi(l)$ is in block $B_m$ and $proj_{\pi'}(l')$ is in block $B'_m$, and $proj_\pi(l)$ is in the same block as $proj_\pi(l+1)$, conclude that $proj_\pi(l+1)$ is in block $B_m$ and  $proj_{\pi'}(l')$ is in block $B'_m$.\note{rewrite using 'block' notation}
%Similarly, before step 3b) suppose the integers maintained are $l,l'$ and so after they are $l+1,l'+t$. By assumption $proj_{\pi}(l+1)$ is in block $B_{m+1}$ and by construction $proj_{\pi'}(l'+t)$ is in block $B'_{m+1}$. 
%
%
%, to show that it is enough to In step 1) since the token did not move and the none of the $g_i$s or $g'_i$s change their local states, the inductive invariant holds. In step 2) the token did not move and the local state of $g'_i$ is the same as that of $g'_i$ ($i \leq k$), the inductive invariant holds. In step 3a) none of the $g_i$s changed local state (since then $proj_\pi(l)$ and $proj_\pi(l+1)$ would be in different $B$-blocks), and the token moved within the same $B$-block and nodes in the same block are $\dminoneCTLstarmX$-equivalent. In step 3b) the nodes in $f_1 \cdots f_{t-1}$ are all equivalent to $\pi_{l}$ since none of the $g'_i$s change state and the token moves within the same block $B'_m$. Also node $f_t$ is equivalent to $\pi'_{l+t}$ since $\token(f_t)$ and $\token(\pi_{l+1})$ are in the same $B$-blok and thus are $\dminoneCTLstarmX$-equivalent by assumption. This completes the verification of the construction, and the inductive step.




%\begin{lemma}
%$P^G \models Q_1 x_1 \cdots Q_k x_k \, \phi$ if and only if $Q_1 x_1 \cdots Q_k x_k \, P^G|{\{x_1,\cdots,x_k\}} \models \phi$.
%\end{lemma}
%
%\begin{proof}
%...
%\end{proof}

\ifblack
{\color{black!40}

...one often gives a computable reduction to a finite set of finite-state model checking problems. This is formalised as follows.

A {\em decomposition} for $(\Pproctemp, \Pgraph,\Pspec)$ is a computable function mapping every triple $(\Pproctemp,\pgraph,\pspec) \in  \Pproctemp \times \Pgraph \times \Pspec$
 to a pair $(\MC_{\sf fin},\Phi_\bbB)$ where:
  
\begin{itemize}
  \item $\MC_{\sf fin}$ is a set
    $\{(K_1,\phi_1),\ldots,(K_m,\phi_m)\}$,  %of size $m$ 
where each $K_i$ is a topology and each $\phi_i$ is a formula, and
 \item $\Phi_\bbB$ is a Boolean formula $\Phi_\bbB(x_1,\ldots,x_m)$
   (with $m$ variables)
\end{itemize}
  
such that, letting $c_i = \top$ iff  $P^{K_i} \models \phi_i$, the following are equivalent:
\begin{enumerate}
\item $\forall n \in \mathbb{N}, P^{\pgraph(n)} \models \pspec(n)$,
\item $\Phi_\bbB(c_1,\ldots,c_m)$ evaluates to $\top$,
\end{enumerate}

Thus a decomposition reduces the problem $\textsf{PMCP}(\Pproctemp, \Pgraph, \Pspec)$ to a Boolean combination of finitely many model checking problems of finite LTSs. For example see Section~\ref{sec:decCTTV}.


%Suppose, as is usually the case, that it is decidable, given a $\numt$-ary topology $G$, $\numt$-ary system template $\systemp$, and a parameterized-specification $\varphi$, whether or not $\overline{P}^G \models \varphi$.
%Then the existence of a computable reduction for $(\Psystemp, \Pgraph,\Pspec)$ implies that the PMC problem for 
%$\Psys$ and $\Pspec$ is decidable where $\Psys$ consists of all parameterized-systems of the form $n \mapsto \systemp^{\pgraph(n)}$ for $\systemp \in \Psystemp$ and $n \mapsto \pgraph(n) \in \Pgraph$.



	We identify a special case of this definition that appears in the literature:
	If $\MC_{\sf fin} = \left\{\left(\pgraph(1),\pspec(1)\right),\ldots,\left(\pgraph(m),\pspec(m)\right)\right\}$
and $\Phi_\bbB = x_1 \land \ldots \land x_m$, we say \emph{$m$ is a cutoff} for
$(\Pproctemp, \pgraph, \pspec)$. 
	If the cutoff is independent of the system template $\Pproctemp$, we say it is a cutoff for $(\pgraph,\pspec)$. 
	
	For example, by the results in Sect.~\ref{sec:decEN}, $2$ is a cutoff for $(\pring,\forall x.\phi)$, where $\pring$ are the rings, and $\forall x. \phi$ is a $1$-indexed  \LTLmX\ formula.\note[SR]{Add that this is for token rings}
	}
	\fi
	
	
	
	
%\section{Cutoffs for \piCTLstarmX\ and fragments}
%\label{sec:decPiCTL}

\subsection{Finiteness Theorem} \label{section:finiteness}


%\begin{reptheorem}{thm:contraction}
%There is an algorithm that given $k,d$ and $(G,x,\bar{g})$ (where $\bar{g}$ is a $k$-tuple over $V_G$, and $x \in V_G$) returns a LTS $\G_{d,\bar{g},x}$ such that
%$\tokengraph{G}{x}{\bar{g}} \equiv_{\dCTLstarmX} \G_{d,\bar{g},x}$. Moreover, for fixed $k,d$ there are finitely many LTSs of the form $\G_{d,\bar{g},x}$ as $G,x,\bar{g}$ vary.
%\end{reptheorem}

\begin{reptheorem}{thm:contraction}
There is an algorithm that given positive integers $k,d$, topology $G$ with initial state $x$, $k$-tuple $\bar{g}$ over $V_G$, returns a LTS $\dcon{G}{x}{\bar{g}}$ such that
$\tokengraph{G}{x}{\bar{g}} \equiv_{\dCTLstarmX} \dcon{G}{x}{\bar{g}}$. Moreover, for fixed $k,d$ there are finitely many LTSs of the form $\dcon{G}{x}{\bar{g}}$ as $G,\bar{g},x$ vary.
\end{reptheorem}

As an immediate corollary we get:
\begin{reptheorem}{thm:finiteness}[\textbf{Finiteness}]
For all integers $k$ and $d$, there are finitely many equivalence classes $[\tokengraph{G}{x}{\bar{g}}]_{\equiv_{\dCTLstarmX}}$ where $G$ is an arbitrary topology, $x \in V_G$ and ${\bar{g}}$ is a $k$-tuple over $V_G$.
\end{reptheorem}


\subsubsection{Proof that i) $(G,x)|\bar{g} \equiv_{\dCTLstarmX} \dcon{G}{x}{\bar{g}}$ and ii) there are finitely many $d$-contractions.}

In order to bound the number of $d$-contractions we need to bound the number of $\sim_d$-equivalence classes. We do this by constructing a finite partial order $(M_d,\preceq_d)$, that only depends on $k$ and $d$, and proving that for all $v$ we have $\mu_d(v) \in M_d$.

Before we begin, we state an easy lemma and some notation.
\begin{lemma} \label{lem:destutw}
If $\destut(w) = \destut(w')$ then there exist partitions $A_1, A_2, \cdots, A_n$ of $[|w|]$ and $A'_1,A'_2, \cdots, A'_n$ of $[|w'|]$ such that for every $i \in \mathbb{N}$ if $j \in A_i$ and $j' \in A'_i$ then $w_j = w'_{j'}$.
\end{lemma}

{\em Notation.} Define $pos_i(w)$ as the largest index $j$ such that $\destut(w_1 \cdots w_j) = \destut(w)_1 \cdots \destut(w)_i$. Intuitively, $pos_i(w)$ is the largest position in $w$ that corresponds to the $i$th letter in $\destut(w)$. Define $pos_0(w) = 0$.  

\paragraph{Definition of $\preceq$}
For sets of strings $X,Y$ define $X \preceq Y$ if for all $x \in X$ there exists $y \in Y$ such that $x$ is a (not necessarily proper) suffix of $y$.

Note $2$. The following {\em monotonicity property} is useful: if $u$ is reachable from $v$ in $G$ then $\mu_{d-1}(u) \preceq \mu_{d-1}(v)$. To prove this take a word $w$ in $\mu_{d-1}(v)$. We know $w = \destut(\pi')$ for some path $\pi'$ starting in $u$. Since $u$ is reachable from $v$ there is a path $\pi$ in $G$ starting in $v$ that has $\pi'$ as a suffix. By the definition of $\destut$, observe 
that $\destut(\pi')$ is a suffix of $\destut(\pi) \in \mu_{d-1}(v)$, as required.

\begin{lemma} \label{lem:sim}
If $u,v \in V_G$ are $\sim_d$-equivalent then $u \equiv_d v$.\note{be more precise, say what $M,N$ are}
\end{lemma}

\begin{proof}
By induction on $d$. The case $d = 0$ is immediate from the definitions. Suppose the result holds for $d-1$. Let $u,v \in V_G$ with $u \sim_d v$. To show $u \equiv_d v$ take a path $\pi$ \note{where is $\pi$?} starting at $u$ (the other case is symmetric).\note{we assume for now that $\pi$ hits $\bar{g}$ infinitely often.} We show that there exists a path $\pi'$ starting at $v$ and paritions $A_1 A_2 \cdots $ of $\pi$ and $B_1 B_2 \cdots$ of $\pi'$ such that for all $i$, if $a \in A_i, b \in B_i$ then $a \equiv_{d-1} b$.


We construct $\pi'$ step by step as follows. Throughout the construction we maintain integers $l,l'$ satisfying the following invariants $(\dagger)$:
\begin{itemize}
\item[i.] the first $l$ elements of $\pi$ have been considered and assigned to blocks $A_1,A_2,\cdots, A_n$ (for some $n$);
\item[ii.] the first $l'$ elements of $\pi'$ have been defined and have been assigned to blocks $A'_1,\cdots, A'_n$;


\item[iii.] $\pi_l \sim_d \pi'_{l'}$;

\item[iiv.] for all $j \leq n$ and $a \in A_j, a' \in A'_j$ we have $\pi_a \equiv_{d-1} \pi'_{a'}$;

\end{itemize}


Initialize with $l = l' = 1$ and $A_1 = A'_1 = \{1\}$. 

Let $t$ be the smallest integer such that $\pi_{l+t}\in \bar{g}$, say $g_j$. Form string $s = \destut(e)$ where $e = \pi_{l+1} \cdots \pi_{l+t}$. Note that $s \in \mu_{d}(\pi_l)$. By invariant iii. $s \in \mu_d(\pi'_{l'})$. Thus there exists a finite path $f = f_0 \cdots f_m$ from $\pi'_{l'}$ to $g_j$, such that $\destut(f) = s$. Append $f_1 \cdots f_m$ to $\pi'$.

For $1 \leq i \leq r$ between $1$ and the length of $s$, form a new block $A_{n+i}$ to include $l+pos_{i-1}(e)+1, \cdots, l+pos_{i}(e)$, and a new block $A'_{n+i}$ to include $l'+pos_{i-1}(f)+1, \cdots, l'+pos_{i}(f)$.


Aside. As long as $\pi$ contains infinitely many elements from $\bar{g}$, $\pi'$ is an infinite path. Otherwise we need to slightly ammend the construction.

This ends the construction. We prove the invariants hold. 

After initialization, the first three invariants are immediate. For the fourth: recall that invariant iii. implies $\pi_l \sim_{d-1} \pi'_{l'}$, and by the induction hypothesis $\pi_l \equiv_{d-1} \pi'_{l'}$.

Suppose we are at the beginning of a step with integers $l,l'$. The first two invariants are immediate by construction. For the third note that  $\pi_{l+t} = g_j = \pi'_{l'+m}$ and $g_j \sim_d g_j$ (reflexivity).

For the fourth invariant observe that by construction for $1 \leq i \leq |s|$ and $a \in A_{n+i}$ and $a' \in A'_{n+i}$ we have that $\mu_{d-1}(a) = s_i = \mu_{d-1}(a')$. Thus by the inductive hypothesis $a \equiv_{d-1} a'$ as required.
\end{proof}

%Let $n_0 := 0$ and let $n_1 < n_2 < n_3 <  \cdots$ be the sequence of positions of $\pi$ such that $\pi_{n_i} \in \bar{g}$.
%%Define $C_i := \{n_i + 1, n_i + 2, \cdots, n_{i+1} - 1\}$. 
%Define partition $A_{2i-1}$ to be $\{n_{i-1}+1, n_{i-1} + 2, \cdots, n_{i} - 1\}$. Define $A_{2i} := \{n_{i}\}$. Note that $A_{2i-1}$ might be empty, but for ease of exposition we will ignore this.\note{clean up}




\paragraph{Definition of $(M_d,\preceq_d)$.}
Define a finite set $M_d$ of finite strings and a partial order $\preceq_d$ on $M_d$.

Define $M_0 := \{1,2,\cdots,k\} \cup \{\emptyset, \bot\}$ and $i \preceq_0 \emptyset$ for $i \in [k] \cup \{\bot\}$ and the others are incomparable. \note{treating $\emptyset$ as a letter might be confusing}

Suppose $M_{d-1}$ is a finite set of finite strings and $\preceq_{d-1}$ is a partial order on $M_{d-1}$.
Define $N_d$ to be the set of decreasing chains in $(M_{d-1},\preceq_{d-1})$. \note{need to add bottom to chain} In other words, $N_d$ is the set of all strings of the form $w_1 \cdots w_t$ such that $w_{i+1} \prec_{d-1} w_i$. Note that $N_d$ is finite.\note{flesh out} Define $M_d$, contained in the powerset of $N_d$, such that $X \in M_d$ iff all strings in $X$ start with the same letter, say $first(X)$.  The partial order $\preceq_d$ on $M_d$ is defined as follows: for $X,Y \in M_d$, define $X \preceq_d Y$ if for all $x \in X$, there exists $y \in Y$ such that $x$ is a suffix of $y$.

To see that $(M_d,\preceq_d)$ is in fact a partial order we check asymmetry (reflexivity and transitivity are trivial). Suppose $X \neq Y$ but $X \preceq_d Y$ and $Y \preceq_d X$. Take a word $first(X) \cdot w \in X \setminus Y$. Since $X \preceq_d Y$ and $first(X) \cdot w \not\in Y$ there exists a possibly empty word $w'$ such that $first(Y) \cdot w' \cdot first(X) \cdot w \in Y$. Since $Y \preceq_d X$ there exists a word $w''$ (possibly empty) such that $u :=  w'' \cdot first(Y) \cdot w' \cdot first(X) \cdot w \in X$.  But $u$ is a decreasing chain in $(M_{d-1},\preceq_{d-1})$, and thus every letter, in particular $first(X)$, appears in $u$ at most once. This is a contradiction since $first(X)$ appears in the following two disjoint substrings of $u$: the non-empty prefix $w'' \cdot first(Y)$, and the suffix $first(X) \cdot w$.


\paragraph{Finitely many $d$-contractions.}
For all $v$ we have $\mu_d(v) \in M_d$, i.e., all strings in $\mu_d(v)$ start with the same letter, and are decreasing chains in the partial order $(M_{d-1},\preceq_{d-1})$. By definition all strings in $\mu_d(v)$ start with $\mu_{d-1}(v)$. For the second, suppose by induction that $\mu_{d-1}(v) \in M_{d-1}$. We want to show that every $w \in \mu_d(v)$ is a decreasing chain in $(M_{d-1},\preceq_{d-1})$. But this follows from monotonicity.


Since we can bound the size of $M_d$ by a function of $k,d$, conclude that the number of nodes in the $d$-contraction is also bounded by this function of $k,d$. Thus, for each $k,d$ there are finitely many $d$-contractions.\note{Compute bound}

\paragraph{$\tokengraph{G}{x}{\bar{g}}$ is $\equiv_d$-equivalent to $ \dcon{G}{x}{\bar{g}}$.}

For $0 \leq j \leq d$ define $\mu_j([u]_{\sim_d}) := \mu_j(u)$, and recall that by Lemma~\ref{lem:refines}. $\mu_j([u]_{\sim_d})$ is independent of the representative $u$.

We prove by induction on $j$ with $0 \leq j \leq d$ that for every $v,w$ in $V_G$, if $\mu_j(v) = \mu_j([w]_{\sim_d})$ it holds that $v \equiv_j [w]_{\sim_d}$. In particular, since $\mu_d(x) = \mu_d([x]_{\sim_d})$ we get that $x \equiv_d [x]_{\sim_d}$ as required.

For $j = 0$. By definition $v$ and $[v]$ have the same label so they are $\equiv_0$ equivalent.

Suppose the result holds for $j < d$, we prove it for $j+1$. Suppose  $\mu_{j+1}(v) = \mu_{j+1}([w]_{\sim_d})$. There are two directions. 

{\em First direction:} let $\pi = \pi_1 \pi_2 \cdots$ be a path in $G$ starting in $v$, and let $w \in V_G$ be a vertex such that $\mu_{j+1}(v) = \mu_{j+1}([w]_{\sim_d})$. In particular $\mu_{j+1}(v) = \mu_{j+1}(w)$. By Lemma~\ref{lem:sim}, $v \equiv_{j+1} w$ and so there is a path $\pi' = \pi'_1 \pi'_2 \cdots$ in $G$ starting in $w$ and partitions $A_1, A_2, \cdots$ of $\pi$ and $A'_1, A'_2, \cdots$ of $\pi'$ such that for all $i$ and $a \in A_i, a' \in A'_i$ we have $\pi_a \equiv_{j} \pi'_{a'}$. Define the sequence $\rho = [\pi'_1]_{\sim_d} [\pi'_2]_{\sim_d} \cdots$ in the contraction. It is immediate that this sequence is a path in the contraction since (for $i \in \Nat$) the edge from $\pi'_i$ to $\pi'_{i+1}$ in $G$ implies, by definition of the edges in the $d$-contraction, that there is an edge from $[\pi'_i]_{\sim_d}$ to $[\pi'_{i+1}]_{\sim_d}$.  Define partitions $B$ of $\rho$ by $B_i := A'_i$ (for $i \in \Nat$). The fact that $\mu_j(\pi'_i) = \mu_j([\pi'_i]_{\sim_d})$ means we can apply the inductive hypothesis to get $\pi'_{i} \equiv_{j} [\pi'_{i}]_{\sim d} = \rho_i$ (for $i \in \Nat$). To finish consider $a \in A_i$ and $b \in B_i$ (for some $i \in \Nat$). Suppose $b = \rho_r$ ($r \in \Nat$). Then $\pi_a \equiv_j \pi'_r$ since $\pi'_r \in A'_i$. So $\pi_a \equiv_j \rho_r$ as required.

For the other direction we start with a lemma.

Lemma. Suppose $[y_1]_{\sim_d} [y_2]_{\sim_d} \cdots [y_r]_{\sim_d}$ is a path in $\dcon{G}{x}{\bar{g}}$ such that $y_r \in \bar{g}$.  For $0 \leq j < d$ the word 
\[
\destut(\mu_{j}(y_1) \mu_{j}(y_2) \cdots \mu_{j}(y_r))
\]
is in $\mu_{j+1}(y_1)$.\note{Rewrite or Point out it is well-defined since equivalent nodes agree}

The proof of the lemma is by induction on the length $r$ of the path. Immediate for $r = 1$ and $0 \leq j < d$ by the definition of $\mu_{j+1}$ and using the fact that $y_r \in \bar{g}$. Suppose the result holds for a path of length $r$. We prove it for a path of length $r+1$. Say $0 \leq j < d$. Take such a path  $[y_1]_{\sim_d} [y_2]_{\sim_d} \cdots [y_{r+1}]_{\sim_d}$. By the induction hypothesis, $s = \destut(\mu_{j}(y_2) \mu_{j}(y_2) \cdots \mu_{j}(y_{r+1}))$ is in $\mu_{j+1}(y_2)$. The edge from $[y_1]_{\sim_d}$ to $[y_2]_{\sim_d}$ implies that there is an edge in $G$ from $z_1$ to $z_2$ for some $z_i \in [y_i]_{\sim_d}$.  Note that since $\sim_d$ refines $\sim_{j+1}$ we get $ \mu_{j+1}(y_i) = \mu_{j+1}(z_i)$ for $i \in \{1,2\}$. Since $s \in \mu_{j+1}(y_2) = \mu_{j+1}(z_2)$ there is a  path $z_2 z_3 \cdots z_m$ in $G$ starting in $z_2$ such that $s = \destut(\mu_j(z_2) \cdots \mu_j(z_m))$. It follows that $\mu_{j+1}(y_1) = \mu_{j+1}(z_1)$ contains the word 
\begin{eqnarray*}
\destut(\mu_j(z_1) \mu_j(z_2) \cdots \mu_j(z_m)) &=& \destut(\mu_j(z_1) s)\\
& =& \destut(\mu_j(y_1) s)\\
& =& \destut(\mu_{j}(y_1) \mu_{j}(y_2) \cdots \mu_{j}(y_{r+1})),
\end{eqnarray*}

where the second equality is since $\mu_{j}(y_1) = \mu_{j}(z_1)$, and the other two are because $\destut(\alpha \cdot \destut(\beta)) = \destut(\alpha \cdot \beta)$ for strings $\alpha,\beta$. 
This completes the proof of the lemma.

{\em Second direction:} Let $\pi' = [y_1]_{\sim_d} [y_2]_{\sim_d} \cdots$ be a path in $\dcon{G}{x}{\bar{g}}$,  and let $v \in V_G$ be a vertex such that $\mu_{j+1}(v) = \mu_{j+1}([y_1]_{\sim_d})$.


As usual we segment $\pi'$. We describe the first segment. Suppose $r$ is the smallest integer such that no element in any of the classes $[y_1]_{\sim_d}, \cdots, [y_{r-1}]_{\sim_d} $ contains a node from $\bar{g}$ \note{make clearer} and $[y_r]_{\sim_d}$ does contain a node from $\bar{g}$. Then by the lemma \note{which?} $s := \destut(\mu_{j}(y_1) \mu_{j}(y_2) \cdots \mu_{j}(y_r))$ is in $\mu_{j+1}(y_1) = \mu_{j+1}(v)$. Thus there is a path $\pi_1 \cdots \pi_m$ in $G$ starting in $v$ such that $\destut(\mu_j(\pi_1) \cdots \mu_j(\pi_m)) = s$.  By Lemma~\ref{lem:destutw} there exist partitions $A_1, \cdots, A_n$ of $[r]$ and $A'_1,\cdots, A'_n$ of $[m]$ such that for $i \leq n$ and $t \in A_i, t' \in A'_i$ it holds that $\mu_j(y_t) = \mu_j(\pi_t)$. 

The last nodes $y_r$ and $\pi_m$ are in $\bar{g}$, and $\mu_j(y_r) = \mu_j(\pi_m)$. Thus in particular $\mu_0(y_r) = \mu_0(\pi_m)$ (by Lemma~\ref{lem:refines}.), and so by definition of the labeling function $\Lambda$ of $G$, we must have $y_r = \pi_m$. But then $\mu_{j+1}([y_r]_d) = \mu_{j+1}(\pi_m)$ and we can continue with the next segment as we did with the first. \qed





%We assume that $\pi'$ does not stutter --- it may since the $d$-contraction may have self loops --- since otherwise we may replace $\pi'$ with $\destut(\pi')$. Define the sequence $\pi = y_1 y_2 \cdots$ where $y_i$ is any representative of the $\sim_d$-equivalence class $\pi'_i$. We first show that $\pi$ is a path in $G$. Observe that it is enough to show that for every $i$ and $y \in \pi'_i$ there is some $z \in \pi'_{i+1}$ and an edge from $y$ to $z$ in $V_G$.


%
%
%At every stage, given $\mu_d$, the $d$-contraction is the LTS whose nodes are 




% \begin{conjecture}
% For all integers $k,d$ and every $\pgraph$, $\PMCP_\pgraph(\Psimptok,\dkCTLstarmX)$ is decidable.
% \end{conjecture}

% The proof sketch unifies ideas from CTTV and EN.

%\begin{lemma}[Composition]
%Fix $k,d$ and let $G,H$ be $k$-graphs. If $G$ and $H$ agree on $\dkCTLstarmX$ formulas then for all $P$, $P^G$ and $P^H$ agree on all $\dkCTLstarmX$ formulas.
%\end{lemma}
%
%\begin{lemma}[Finiteness]
%Fix $k,d$. There exists finitely many $k$-graphs $H_1,\cdots,H_l$ such that for every $k$-graph is $\dkCTLstarmX$ there exists $i \leq l$ such that $G$ is equivalent to some $H_i$.
%\end{lemma}

\ifblack


{\color{black!30}



Define a $d$-round game between LTSs $G,H$ such that Duplicator has a winning strategy if and only if $G$ and $H$ agree on all $\dCTLstarmX$ formulas. Suppose $\left<(G^0,g_0^0),(G^1,g_0^1)\right>$ is the current position. A round proceeds in two phases. In the first phase Spoiler pick a structure, say $G^i$, and an infinite path starting in $g^i_0$, then Duplicator responds with an infinite path in the other structure, $G^{1-i}$, starting in $g^{1- i}_0$, resulting in position $\left<(G^0,\pi^0,g_0^0),(G^1,\pi^1,g_0^1)\right>$. This is the end of the first phase. The second phase consists of a number of subphases --- the total number is determined by Spoiler. Suppose after the $j$th subphase the position is $\left<(G^0,\pi^0,g^0_j),(G^1,\pi^1,g^1_j)\right>$. In the next subphase Spoiler picks a point $g^i_{j+1}$ on one of the paths $\pi^i$ and Duplicator responds with a point $g^{1-i}_{j+1}$ on the other path so that a) $g^0_{j+1}$ and $g^1_{j+1}$ have the same label and b) $g^0_j$ is before $g^0_{j+1}$ on path $\pi^0$ iff $g^1_j$ is before $g^1_{j+1}$ on path $\pi^1$ (in each subphase Spoiler may pick a point from either path). To finish the second phase Spoiler stops picking points, say after $m$ steps, and the new position is $\left<(G^0,g^0_m),(G^1,g^1_m)\right>$. This completes the round. If at any stage along a play Duplicator is unable to respond then we say that Duplicator does not survive that round. Duplicator wins a play if she survives the first $d$ rounds. %The proof of the following lemma is standard, see \cite{}.

\begin{lemma}
For every $G,H$, and integer $d$, Duplicator has a winning strategy in the $d$-round game described above if and only if $G$ and $H$ agree on all $\dCTLstarmX$ formulas.\note{Actually, this needs to be checked}
\end{lemma}

}

\fi





==> DetailedDfns.tex <==
\section{Detailed Definitions} \label{app:detdfns}

\subsubsection*{$\CTLstar$}
Here is a brief description of the the syntax and semantics of $\CTLstar$, see for instance \cite{PrinciplesMC}.

\paragraph{Syntax}

The syntax of $\CTLstar$\ over a set $\AP$ of atomic propositions is defined as follows.

\emph{State formulae} are formed according to the grammar:
\[
\Phi ::= \top  \vsp   
p \vsp 
\Phi \wedge \Psi  \vsp  
\neg \Phi \vsp 
\ctlE \varphi
\]
where $p \in \AP$ and $\varphi$ is a path formula and 
$\Phi,\Psi$ are state formulae.

\emph{Path formulae} are formed according to the grammar:
\[
\varphi ::= \Phi \vsp 
\varphi \wedge \psi \vsp 
\neg \varphi \vsp 
\varphi \ltlU \psi \vsp 
\ltlX \varphi
\]
where $\Phi$ is a state formula and $\varphi,\psi$ are
path formulae. From these we derive, as usual, Boolean operators (like
$\vee$), temporal operators  $\ltlF$ (eventually) and  $\ltlG$ (always), and the universal path quantifier $\ctlA$.

\paragraph{Semantics}
Formulas are interpreted in LTSs $M = (Q,Q_0,\delta,\lambda)$ over atomic propositions $\AP$. The semantics for Boolean operations are defined as usual, see \cite{PrinciplesMC}.

For state $s$ of $M$, define i)
$(M,s) \models p$ iff $p \in \lambda(s)$, and ii)
%(M,s) \models \neg \Phi & \iff \text{not} (M,s) \models \Phi\\
%(M,s) \models \Phi_1 \wedge \Phi_2 & \iff (M,s) \models \Phi_1 \text{ and } (M,s) \models \Phi_2\\
$(M,s) \models \ctlE \varphi$ iff $(M,\pi) \models \varphi$ for some infinite path $\pi$ of $M$ starting in $s$.

For infinite path $\pi$ of $M$ starting in $s$, write $\pi^j$ for the path $\pi$ starting at position $j \geq 0$.
Define i) $(M,\pi) \models p$ iff  $(M,s) \models p$, ii) $(M,\pi) \models \ltlX \varphi$ iff $(M,\pi^1) \models \varphi$, and iii)  $(M,\pi) \models \varphi \ltlU \psi$ iff $(\exists j \geq 0) (\forall k < j) \left[(M,\pi^j) \models \psi \wedge (M,\pi^k) \models \varphi\right]$.

Define $M \models \phi$ if for every\note{check this choice} initial state $q \in Q_0$, $(M,q) \models \phi$.

\subsubsection*{\dCTLstarmX}

We identify important syntactic fragments of \CTLstar. Let \CTLstarmX\ be the syntactic fragment of \CTL\ in which \ltlX\ is not used. For every integer $d$, define \dCTLstarmX\ to be the syntactic fragment in which path quantifiers $\ctlA$ and $\ctlE$ are nested at most $d$ times~\cite{SKS}. 

\paragraph{Syntax} 
The syntax of $\dCTLstarmX$ is defined inductively on $d$.
Write $\Phi_d,\Psi_d$ for $\dCTLstarmX$ state formulae, 
$\varphi_d,\psi_d$ for $\dCTLstarmX$ path formulae,
$p\in \AP$.

Start with $d=0$. 
The $\xCTLstarmX{0}$ state formulae are defined as:
\[
\Phi_0 ::= \top  \vsp  p  \vsp  \Phi_0 \wedge \Psi_0  \vsp  \neg \Phi_0 
\]
and the $\xCTLstarmX{0}$ path formulae are defined as:
\[
\varphi_0 ::= \Phi_0  \vsp  
            \varphi_0 \wedge \psi_0  \vsp   
            \neg \varphi_0  \vsp 
            \varphi_0 \ltlU \psi_0 .
\]

The $\xCTLstarmX{d+1}$ state formulae are defined as:
\[
\Phi_{d+1} ::= 
         \Phi_d  \vsp  
         \Phi_{d+1} \wedge \Psi_{d+1}  \vsp  
         \neg \Phi_{d+1} \vsp
         \ctlE \varphi_d  
\]
and the $\xCTLstarmX{d+1}$ path formula are defined as:
\[
\varphi_{d+1} ::= \varphi_d \vsp 
            \Phi_{d+1}   \vsp  
            \varphi_{d+1} \wedge \psi_{d+1}  \vsp  
            \neg \varphi_{d+1}  \vsp 
            \varphi_{d+1} \ltlU \psi_{d+1}  .
\]
From these we derive Boolean operators (like $\vee$), 
temporal operators $\ltlF$ (eventually) and $\ltlG$ (always), 
and the universal path quantifier $\ctlA$.

Thus, $\xCTLstarmX{1}$ formulae are Boolean combinations of $\LTLmX$ formulae\footnote{Note the negation of $\LTLmX$ is not necessary an $\LTLmX$ formula.},
for example: $\ctlE (p \ltlU q) \land \ctlA \ltlG\neg (p\land q)$. 
An example of $\xCTLstarmX{2}$ formula is 
$\ctlE (p \ltlU \EG(p\land q))$.

\paragraph{Semantics}
Since $\dCTLstarmX$ is a syntactic fragment of $\CTLstarmX$, the semantics are the same.

\paragraph{Characterization}
The following characterization of \dCTLstarmX, taken from \cite{SKS}, is central to our proofs of the reduction and finiteness theorems.

\begin{definition}
A {\em partition} of a\ak{infinite?} path $\pi$ is an infinite sequence $B_1, B_2, \cdots$ of nonempty disjoint finite sets of states such that $\pi_1 \in B_1$ and for $i \geq 1, j \geq 2$, we have that $\pi_{i+1} \in B_j$ iff either $\pi_i \in B_j$ or $\pi_i \in B_{j-1}$.
\end{definition}

\begin{definition} \label{dfn:equiv}
For LTSs $M,M'$ (with labeling functions $L,L'$ over the same set of atomic propositions) and integer $d$ define relations $\equiv_d \subset M \times M'$ as follows. For states $s$ from $M$ and $s'$ from $M'$, define
\begin{enumerate}
\item $s \equiv_0 s'$ if $L(s) = L'(s')$; and
\item $s \equiv_{d+1} s'$ if for every path $\pi$ in $M$ from $s$ there exists a path $\pi'$ in $M'$ from $s'$ (and vice versa) and a partition $B_1B_2\cdots$ of $\pi$ and a partition $B'_1 B'_2 \cdots$ of $\pi'$ such that for every $i \in \Nat$ and every $t \in B_i, t' \in B'_i$ we have that $t \equiv_d t'$.
\end{enumerate}
\end{definition}

Note that if $s \equiv_{d+1} s'$ then $s \equiv_d s'$, and that in $2.$ we have that if $s$ and $t$ are both in block $B_i$ then they have the same label since $s \equiv_0 \pi'_j \equiv_0 t$ for every $j$ in $B'_i$.

\begin{proposition}\label{prop:equiv} \cite[Theorem $4.2$]{SKS}
For integer $d$, LTSs $M,M'$, and states $s,s'$: The systems $(M,s)$ and $(M',s')$ agree on all \dCTLstarmX\ formulas if and only if $s \equiv_d s'$.
\end{proposition}

\subsubsection*{Indexed Temporal Logic}

\paragraph{Semantics} Indexed-$\CTLstar$\ formulas are interpreted over
a system instance $P^G$ (with $P$ a process template and $G =
(V_G,E_G)$ a topology) as follows. A {\em valuation of the
  variables} is a function $e:\VarNames \to \Nat$. An
\emph{$x$-variant} of $e$ is a valuation $e'$ with $e'(y)=e(y)$ for
all $y \in X \setminus {x}$. 

For state
formula $\varphi$ define $(P^G,e,s) \models \phi$ inductively (path
formulas are interpreted similarly, but over $(P^G,e,\pi)$ where $\pi$
is an infinite path). The only new cases are the base case, the
quantifier cases, the $x = y$ case, and the $x \in E(y)$ case.
\begin{itemize}
\item Define $(P^G,e,s) \models p_x$ to mean that $p_{e(x)} \in
\Lambda(s)$. 
\item Define $(P^G,e,s) \models \forall x. \varphi$ to mean
that for all $x$-variants $e'$ of $e$ it holds that $(P^G,e',s)
\models \phi$. 
\item Define $(P^G,e,s) \models x = y$ to mean that $e(x) = e(y)$.
\item Define $(P^G,e,s) \models x \in E(y)$ to mean that $(e(y),e(x)) \in E_G$ where $E_G$ is the edge relation of $G$.

\end{itemize}

An atom $p_x$ or variable $x$ in an indexed-$\CTLstar$\ formula is {\em bound} if
it is in the scope of a quantifier $\forall x$.
An indexed-$\CTLstar$\ formula $\varphi$ is a {\em sentence} if every atom in it is bound; in this case define $(P^G,s) \models \varphi$ if for all evaluations (equivalently, for some evaluation) $e:\VarNames \to \Nat$, it holds that $(P^G,e,s) \models \varphi$. Finally define 
\[
P^G \models \varphi
\]
if for every\sr{check this choice} initial state $s$ of $P^G$ it holds that $(P^G,s) \models \varphi$. This completes the definition of Indexed-$\CTLstar$.



{\em Notation.}\sr{not sure this is used anywhere}
Write $\iCTLstar$ for the set of all indexed-$\CTLstar$\ sentences. Writing TL  for the various natural fragments of $\CTLstar$, such as \LTL\ and $\LTLmX$, one can similarly define indexed-TL, e.g., $\iLTLmX$ is the set of indexed-$\LTLmX$\ sentences. \sr{it seems this notation is not used}




==> UndecPrenex.tex <==
\section{Undecidability of \piLTLmX\ and \twoCTLstarmX}
\label{appendix:undecprenex}

\begin{reptheorem}{thm:undecprenex}
There exists a process $P \in \Psimptok$, and parameterized topologies \pgraph, \pgraphH, such that the following PMCP problems are undecidable:
\begin{enumerate}
\item $\PMCP_\pgraph(\{P\},\piLTLmX )$.
\item $\PMCP_\pgraphH(\{P\},\twoCTLmX )$.
\end{enumerate}
\end{reptheorem}

\begin{proof}[Sketch]
%For every integer $n$ let $C_n$ be the graph which is simply a chain of $n$ nodes.
Define $P$ to be the process template with two states: there is a transition from the state with the token to the state without the token, and vice versa. In particular, note that $P$ satisfies the EN-restriction in Definition of process template (Section~\ref{dfn:paramsys}).

For every two integers $i,j$ let $L_{i,j}$ be a lasso with a ring of size $i$, and a tail of length $j$.
\ak{can we change it to Lollipop? ``---()''?
Otherwise (``()---''): either the last process never releases the token
(and violates ENrestriction), or releases, and ``blocks'' making the path finite.}
Fix some computable ordering on all deterministic Turing machines (for example,
lexicographic).

Let $\pgraph$ consist of all the topologies of the form $L_{i,j}$ such that the $i$th Turing machine halts on the empty word in at most $j$ steps.


For every $k \in \Nat$ let $\varphi_k$ be the formula in \kLTLmX\ stating there exists $x_1, \cdots, x_k$, all different, such that there exists a path $\pi$ on which it holds that $x_1$ has the token until $x_2$ has the token until \dots until $x_k$ has the token until $x_1$ has the token. Thus $P^G \models \varphi_k$ if and only if $G$ has, as a subgraph, a ring of size $k$.

Now reduce the non-halting problem for TMs to PMCP: the $n$th TM does not halt iff $\pgraph$ does not contain a graph with a loop of size $n$ iff $P^G \models \neg \varphi_n$ for all $G \in \pgraph$.

The second item can be proved in a similar manner using simple variations on the graphs from \cite[Theorem $5$]{CTTV04}.
\qed \end{proof}



==> UndecProof.tex <==
\section{Proofs of Undecidability for Direction-aware TPSs}\ak{check that the word `path' is not messed with 'run'}
\label{appendix:dir-aware}

\begin{reptheorem}{thm:DA}
There exists a parameterized topology $\pgraph$ such that 
the problem $\PMCP_{\pgraph}(\Psnd,\nineallLTLmX)$
is undecidable.
\end{reptheorem}
% \begin{reptheorem}{thm:NC}
% There exists a parameterized topology $\pgraph$ such that 
% the problem $\PMCP_{\pgraph}(\Psnd,\piLTLmX)$
% is undecidable.
% \end{reptheorem}

\begin{proof}
We reduce the non-halting problem for 2CM to 
$\PMCP_{\pgraph}(\Psnd,\nineallLTLmX)$. 
The idea of the reduction is to build a topology $G$,
formula $F \in \nineallLTLmX$,
and a process template $P$ (that depends on a given 2CM),
such that $P^G$ will simulate a partial run of the 2CM. 
Some of the paths of $P^G$ will not correspond to any paths of the 2CM,
so the formula $F$ will have assumptions to to filter out such paths.
% We first describe parameterized topology $\pgraph$ and then, as usual, 
% given a deterministic 2CM $M$ we build process $P \in \Psnd$ and $\piLTLmX$ formula $\phi$ 
% (in fact, $9$-index LTL with $\ltlF$ and $\ltlG$) 
Hence for all $G \in \pgraph$, $P^{G} \models F$ if and only if 
there is no halting computation of the 2CM. 

\paragraph{Topology $\pgraph$.}
\iffig
\begin{figure}
\centering
\subfigure[Edges used in the simulation of a 2CM.]{%
\input{fig_piltl_ny_undec}
\label{fig:fig_piltl_ny_undec_sim}}
% 
\quad
% 
\subfigure[Edges used in the initialization phase.]{%
\input{fig_piltl_ny_undec_init}
\label{fig:fig_piltl_ny_undec_init}}
% 
\caption{Topology used in the proof of undecidability 
of $\PMCP$ of $\Psnd$ on general graphs wrt. $\nineallLTLmX$
($c\in\{1,2\}$; edges to the sink are not shown, some edge labels are omitted).}
\label{fig:fig_piltl_ny_undec}
\end{figure}

% 
% 
% 
% \begin{figure}
%  \begin{subfigure}[b]{0.49\textwidth}
%     \centering
% %     \resizebox{\linewidth}{!}{
%       \input{fig_piltl_ny_undec}
% %     }  
%     \caption{Edges used in the simulation of a 2CM.}
%     \label{fig:fig_piltl_ny_undec_sim}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.49\textwidth}
%     \centering
% %     \resizebox{\linewidth}{!}{
%       \input{fig_piltl_ny_undec_init}
% %     }  
%     \caption{Edges used in the initialization phase.}
%     \label{fig:fig_piltl_ny_undec_init}
%  \end{subfigure}
% %  
% \caption{Topology used in the proof of undecidability 
% of $\PMCP$ of $\Psnd$ on general graphs wrt. $\nineallLTLmX$
% ($c\in\{1,2\}$; edges to the sink are not shown, some edge labels are omitted).}
% \label{fig:fig_piltl_ny_undec}
% % 
% \end{figure}
\fi
% 
\ak{use different colors for edges of different type.}
\ak{add labels to edges on fig(b)}
% 
The topology structure is shown on Fig.~\ref{fig:fig_piltl_ny_undec}
\footnote{Although parallel edges are not allowed 
by the Definition~\ref{def:graph_with_dir} of topologies with directions, 
they can be emulated via adding auxiliary nodes.}
.
Consider the topology $G \in \pgraph$ with $2n+9$ vertices. 
Informally one vertex is called $con$, and for each $c \in \{1,2\}$ 
there is a vertex called $dec^c, inc^c$, $z^c$ (counter $c$ is zero), 
and $nz^c$ (counter $c$ is non-zero). These 9 vertices are called `non-memory' vertices, 
while the remainder all called `memory' vertices. 
There are $n$ vertices called $m^c_1,\cdots,m^c_n$ that encode counter $c$.
Let $\edge{a}{b}{A}$ mean there is a direct edge from $a$ to $b$ marked with $A$. 
Then edges are as follows:

\begin{itemize}
\item $\edge{con}{m_i^c}{M^c}$ for $i \leq n$,
\item $\edge{m^c_i}{m^c_{i+1}}{M^c}$ for $i < n$, 
\item $\edge{m^c_i}{dec^c}{DEC^c}$ for $i \leq n$,
\item $\edge{m^c_i}{inc^c}{INC^c}$ for $i \leq n$,
\item $\edge{con}{m^c_1}{TZ^c}$,
\item $\edge{m^c_i}{nz^c}{NZ^c}$ for $i \leq n$,
\item $\edge{m^c_n}{z^c}{Z^c}$,
% \item $\edge{inc^c}{con}{INC^c-CON}$,
% $\edge{dec^c}{con}{DEC^c-CON}$, 
% $\edge{nz^c}{con}{NZ^c-CON}$ 
% and $\edge{z^c}{con}{Z^c-CON}$,
\item from each of $inc^c, dec^c, nz^c, z^c$ to $con$. The labels are $INC^c-CON$ etc.,
\item from $con$ to each of $inc^c,dec^c,nz^c$ and $z^c$. The labels are $CON-INC^c$ etc.
\end{itemize}
% The graphs has the following edges labels sets: 
% $\dirset_{\trcv}=\{\epsilon\}$,
% $\dirset_{\tsnd}=\{\lM, \lTZ, \lInc, \lDec, \lZ, \lNZ, 
% \lConDec, \lConInc, \lConNZ, \lConZ, 
% \lDecCon, \lIncCon, \lNzCon, \lZCon, \lZCon\}$.
% The role of these edge labels will become clear below.

On Fig.~\ref{fig:fig_piltl_ny_undec} not all edges are drawn - only important ones
\footnote{From each vertex there is an outgoing edge for each possible edge label,
as required by the definition of a direction-aware topology 
in Section~\ref{sec:DATPS}.}
.   
For instance, there is no edge labelled with $\lZ$ from a vertex called $m^c_1$. 
We omit it to keep the figure readable. 
But each vertex of the topology has an edge for each label in $\dirset_\tsnd$:
if no such edge is drawn, then we assume the edge going from the vertex 
to the special node `sink'. 
The `sink' node is a part of a strongly connected subgraph, 
which goal is to keep the token in it for ever. 
`Sink' is not shown on the figure.

\paragraph{Process $P$.}
The process is built out of $11$ components
\footnote{One could use less components, but we choose these for readability.}
.
When a process first receives the token 
it makes a non-deterministic move to one of these $11$ components. 
The components are called 
`controller',
`memory cell of counter $c$', 
`decrement $c$', 
`increment $c$', 
`zero $c$', 
`non-zero $c$'
for $c \in \{1,2\}$.
Informally the process at the $con$ vertex will enter the `controller' component when first scheduled,
the process at the $inc^c$ vertex will enter `increment $c$' component when first receives the token, 
etc. An initialization phase together with the formula described below will enforce this.

Each of the following components `increment $c$', `decrement $c$', `zero $c$', `non-zero $c$'  
has two states, one with the token, one without, and transitions between them. The transition giving up the token from component, say `increment $c$', sends it along an edge labeled $INC^c-CON$. The labels of the other components are similar. 

The `memory of counter $c$' component stores a binary value $b$ which starts with $b = 0$. 
If a process has $b = 0$ and has the token then that process can either
\begin{itemize}
\item[a)] send the token along the $INC^c$ edge and set $b = 1$, or 
\item[b)] send the token along the $M^c$ edge,  or 
\item[c)] in case the process is $m^c_n$ it can send the token along the $Z^c$ edge.
\end{itemize} 
If a process has $b = 1$ and holds the token then the process can either 
\begin{itemize}
\item[a)] send the token along a $DEC^c$ edge and set $b = 0$, or 
\item[b)] send the token along the $NZ^c$ edge
\end{itemize} 
Note that a memory node with $b = 1$ can not pass the token along an $M^c$ edge to the next memory node. Note that the memory component satisfies the EN-fairness restriction 
as specified in Sec.~{\ref{def:process_template}}. Indeed:
if the process has the token, 
the next time it is involved in a global transition 
it must give up the token; 
and similarly if it does not have the token its only possible move is to receive the token.

The `controller' component executes in two phases.
First is an initialization phase in which 
it sends the token along various edges in order to establish, 
for instance, that the process at vertex labeled $inc^1$ is in component $inc^1$.
Second is the simulation phase. A state of `controller' is a tuple of the form $(cur, action, token)$ where $cur$ is the current state of the 2CM, $token$ takes values from $\{yes,no\}$, and $action$ takes values from
\[
\{init^i: i \in [9]\} \cup \{null, inc^1, dec^1, then^1, else^1, inc^2, dec^2, then^2, else^2\}.
\]

The initial state is $(q_0,init,yes)$.

Initialization phase: the controller behaves as follows. 
From the initial state  
there is the following pipeline of transitions. For each $i \in [9]$, 
from $(q_0,init^i,no)$ there is a transition to $(q_0,init^i,yes)$, and:
\begin{itemize}
\item $(q_0, init^1,yes) \to (q_0,init^2,no)$ that sends along ${CON-INC^1}$ edge.
\item $(q_0, init^2,yes) \to (q_0, init^3,no)$ that sends along ${CON-INC^2}$ edge.
\item $(q_0, init^3,yes) \to (q_0, init^4,no)$ that sends along $CON-DEC^1$ edge.
\item $(q_0, init^4,yes) \to (q_0, init^5,no)$ that sends along $CON-DEC^2$ edge.
\item $(q_0, init^5,yes) \to (q_0, init^6,no)$ that sends along $CON-Z^1$ edge.
\item $(q_0, init^6,yes) \to (q_0, init^7,no)$ that sends along $CON-Z^2$ edge.
\item $(q_0, init^7,yes) \to (q_0, init^8,no)$ that sends along $CON-NZ^1$ edge.
\item $(q_0, init^8,yes) \to (q_0, init^9,no)$ that sends along $CON-NZ^2$ edge.
\end{itemize}

\begin{lemma}[Controller initialization]\label{piltl_nc_undec:init_lemma}
The process $i$ in the controller component can complete its initialization phase
(the process reaches state $(q_0, init^9, yes)$) 
if and only if: 
1) $i=con$, and
2) the processes at vertices $inc^c,dec^c,nz^c,z^c$ on first receiving of the token 
go into corresponding components `increment $c$', `decrement $c$', etc.
\end{lemma}
\begin{proof}
$\Rightarrow$: 
  Suppose 1) doesn't hold. The vertex $con$ is the only one 
  that has connections to all of the vertices $inc^c,dec^c,nz^c,z^c$. 
  Hence if $i \ne con$ then one of the token sendings will go into the `sink' node 
  and the initialization phase will not be completed. Similarly if 2) doesn't hold 
  -- the token will end in the `sink' node.   

$\Leftarrow$ follows from the description of the controller process template.
\qed
\end{proof}
% For instance,
% if the process at vertex $inc^c$ for some $c$ 
% is not in component `increase $c$',
% then the process will send the token along any but $\lConInc$ edge. 
% As a result the token will be sent to a node in a special subgraph called `sink', 
% and will never leave it.

\newcommand{\myedge}[1]{\stackrel{{{#1}}}{\rightarrow}}

If the initialization phase succeeds, the simulation phase starts. 
First, the controller moves from $(q_0,init^9,yes)$ to $(q_0,null,yes)$. 
Then the controller makes the following transitions:
\ak{Mention internal transitions of 2CM.}
\begin{itemize}
\item If the command of the 2CM from state $q$ is \textit{`increment $c$ and goto $q'$'}
then: $(q,null,yes) \myedge{\lM} (q,null,no) \to (q',inc^c,no) \to (q',null,yes)$.
\footnote{We use an intermediate state $(q,null,no)$ between 
$(q,null,yes)$ and $(q',inc^c,no)$, 
so we can build the formula (described later) without $\ltlU$ operator.}

\item Similarly for an \textit{`decrement $c$ and goto $q'$'} command 
except $inc^c$ is replaced with $dec^c$.

\item If the command from $q$ is 
\textit{`if counter $c$ equals zero then goto $q'$ else goto $q''$'}, then: 
$(q,null,yes) \myedge{\lTZ} (q,null,no)$, 
and then the controller guesses the result of zero-check
and goes from $(q,null,no)$:
\begin{itemize}
  \item 
  to $(q',then^c,no) \to (q',null,yes)$,
   and the token should have come from vertex $z^c$, or
  \item 
  to $(q'',else^c,no) \to (q'',null,yes)$,
   and the token should have come from vertex $nz^c$.
\end{itemize}  
We use the formula $\ltlG \ValidRun$ 
(described below) to ensure that the controller's guess is correct, 
that is, 
whenever the controller enters state $(q',then^c,no)$ 
the token will come from vertex $z^c$, etc. 
\end{itemize}

% Note that the 'controller' component satisfies the EN-restriction on processes: 
% a process having the token can only receive it; 
% a process not having the token must receive if it takes at least two local transitions.

\paragraph{Atomic propositions.}\ak{edges must be labelled with textsf or whatever but capitalized -- confusion}
These are, for $c \in \{1,2\}$:
\begin{itemize}
\item $INC^c\_TOK$ which holds  in the `increment $c$' component that has the token;
\item $DEC^c\_TOK$ which holds in the `decrement $c$' component that has the token;
\item $Z^c\_TOK$ which holds  in the `zero $c$' component that has the token;
\item $NZ^c\_TOK$ which holds  in the `non-zero $c$' component that has the token;
\item $CON\_INC^c$ which holds in the states of `controller' that has $action = inc^c$;
\item $CON\_DEC^c$ which holds in the states of `controller' that has $action = dec^c$;
\item $CON\_Z^c$ which holds in the states of `controller' that has $action = then^c$;
\item $CON\_NZ^c$ which holds in the states of `controller' that has $action = else^c$;
\item $HALT$ which holds in controller states of the form $cur = halt$ 
      where $halt$ is the (unique) final state of the 2CM.
\end{itemize}

\paragraph{Formula $F$.}
\label{piltl_undec_nc:formula}
Let $W$ be a variable which varies over elements from the sequence 
$(\Velements)$. 
Let $ord(W) \in [8]$ be the position of $W$ in this sequence, 
e.g., if $W = DEC1$ then $ord(W) = 2$.

The formula $F$ is of the form\ak{try to unfold VALID part of the formula -- easier to read?}
\[
\forall x \forall y_1 \cdots \forall y_8: \,  \ltlG\ValidRun \to \ltlG\neg HALT_x
\]
where 
$\ValidRun = \bigwedge_W  (CON\_W_{x} \to W\_TOK_{y_{ord(W)}})$ 
. Recall that we consider $\nineallLTLmX$ and 
therefore path quantifier $\ctlA$ is right after the index quantifiers. 

Intuitively, ``$\ltlG\ValidRun$ is true'' 
means that during the run all guesses of all processes were correct: 
the controller correctly guessed the results of test for zero operations, 
the memory nodes correctly guessed the commands the controller wants them to execute.
Also, $\ltlG\ValidRun$ is false when the controller doing `increment $c$' sends 
the token to a memory node in state with $b=1$.

\paragraph{Examples.}
Consider how a simulation of an \emph{`increment $c$'} command works.
The controller sends the token along $M^c$ edge 
to a non-deterministically chosen memory node.
If the process at the node is not in the `memory of counter $c$' component,
then it will send the token along any edge but those drawn on the figure for that node, 
and the token will end up in the `sink' node, and $\ltlG \ValidRun$ will be falsified.
If the process is in the `memory of counter $c$' component
and has its $b=0$, 
then it guesses the command to execute: 
\emph{`increase $c$'} or \emph{`test $c$ for zero'}.  
If it guesses the former, then it sets $b=1$ and sends the token to $inc^c$ 
completing the simulation of the command. 
If it guesses \emph{`test $c$ for zero'} then it sends the token along $M^c$ edge.
It is still possible to complete the command if the token end up 
in the memory process with $b=0$ that correctly guesses the command.
Otherwise, the token will be sent to one of $dec^c,nz^c,z^c$
nodes and $\ltlG \ValidRun$ will be falsified. 

Similarly works simulation of \emph{`test $c$ for zero'}. If the controller
guesses `counter $c$ is zero', then in order $\ltlG \ValidRun$ to be true, 
the token should go through all of the memory nodes, which is possible 
only if all the memory nodes have $b=0$ and correctly guess the command.
Note that the memory process having $b=1$ never sends the token along 
$M^c$ edge to the next memory process.

\paragraph{Correctness.}
In previous paragraphs we described how for a given 2CM 
to build a process template $P \in \Psnd$,
a parameterized topology $\pgraph$, and a formula ${F \in \nineallLTLmX}$. 
Here we show that the 2CM doesn't halt if and only if 
the answer to $\PMCP$ for the $P^{\pgraph}$ with respect to the formula $F$ is ``Yes''.

We first describe how \emph{a global state of $P^{G}$} (where $G$ has $2n + 9$ nodes)
\emph{encodes the 2CM configuration} $(q,cnt_1,cnt_2)$ with counter values at most $n$:
\begin{itemize}
  \item the process at node $con$ is in a local state $(q,null,yes)$;
  \item processes at nodes $inc^c,dec^c,z^c,nz^c$ 
  are in a state of a corresponding component and has no token;\ak{picture of processes impl would help}
  \item the processes at nodes $m_i^c$ are in a state of the memory 
  component or are still in the local initial state $\iota$ of the memory component,
  and for each $c \in \{1,2\}$, 
  $cnt_c$ is equal 
  to the number of processes at vertices $m_1^c, \cdots, m_n^c$ having  $b = 1$.
\end{itemize} 
Note: 
a) not every global state of $P^{G}$ encodes a configuration of 2CM, and 
b) there may be more than one encoding of the same configuration 
because a counter value $k>0$ may be encoded 
by any way of having $k$ out of the $n$ processes with $b = 1$.

Second, we describe how \emph{a path $\pi$} of $P^{G}$ 
\emph{encodes an $n$-partial run} $conf_1\ conf_2\ \dots$ of the 2CM
\footnote{An \emph{$n$-partial run} of a 2CM $M$ is a run of a modified 2CM $M'$:
$M'$ is the same as $M$ except when one of counters $cnt_1$ or $cnt_2$ 
reaches the value $n$ then $M'$ loops in some state by doing some internal transition.
Thus: 
1) an $n$-partial doesn't contain a configuration with $cnt_1$ or $cnt_2$ larger than $n$;
2) an $n$-partial run is infinite;
3) a 2CM halts if and only if it has an $n$-partial run which reaches a halting state.
}
.
Let $\pi_{conf}$ be the subsequence of $\pi$ 
consisting of all global states that encode a configuration of the 2CM. 
Let $\pi_{conf}'$ be the subsequence of $\pi_{conf}$ 
formed by deleting from $\pi_{conf}$ consecutive global states 
that encode the same configuration. 
We say that $\pi$ encodes the partial run 
if for all $i$, $\pi_{conf}'[i]$ encodes $conf_i$.

Before proving the correctness result we prove Lemma~\ref{piltl_ny_undec:l3}
and Lemma~\ref{piltl_ny_undec:l1}.
\begin{lemma}[2CM by $P^G$]\label{piltl_ny_undec:l1}
For every $n$, an $n$-partial run of 2CM is encoded by some path $\pi$ in $P^G$ 
  (where $G \in \pgraph$ and has $2n+9$ nodes) 
  that satisfies 
  $\ltlG\ValidRun$ 
  for the following assignment of the index variables: 
  $x = con$ and $y_i = ord^{-1}(i)$, that is, $y_1=inc^1, y_2=dec^1, y_3=z^1$, etc.
\end{lemma}
\begin{proof}[idea] 
Take an $n$-partial run of the 2CM $conf_1\ conf_2\ \dots$. The path is as follows:
the path correspondig to succesfull initialization phase 
followed by a path corresponding to a simulation phase.
The process at vertex $con$ starts in the initial state with the token, 
moves into the controller component initial state $(q_0, init, yes)$.
The process then starts initialization phase. 
There are transitions of processes of $P^G$ that lead to succesfull completion of
the initalization phase (when processes at vertices $inc^c, dec^c, \ldots$ moves into 
components `increment $c$', `decrement $c$', \ldots\ as shown on the Fig.~\ref{fig:fig_piltl_ny_undec}). 

% It then passes the token along the edge labelled $CON-INC^1$. The process at vertex $INC^1$ moves to the 'increment $1$' component and sends the token back along the $INC^1-CON$ edge. The controller repeats this relay with every node $V$ from the rest of the list $(INC2,Z1,Z2,NZ1,NZ2)$. Observe that at the end of this stage the process at node $V$ is in component $V$ for $V \in (INC1,INC2,Z1,Z2,NZ1,NZ2)$ and all the processes at the other nodes are in the initial state. The 'controller' process now moves from $(q_0,init^9,yes)$ to $(q_0,null,yes)$. This completes the initialization phase.

After the initialization phase completes, the controller process (at vertex $con$)
starts a simulation of the 2CM, as written in the description of the process template. 
The idea is this:
\begin{itemize}
  \item Suppose the 2CM says \textit{`increment counter $1$ and goto state $q'$'}. 
The controller sends the token along $M^1$ edge to one of processes in the memory component. 
The formula part $(CON\_INC^1_{con} \to INC^1\_TOK_{inc^1})$ 
of $\ValidRun$ checks that 
when the controller process (at vertex $con$) is scheduled for the next time   
the process in the component `increment $1$' (at vertex $inc^1$) has the token.
This ensures that the increment command was correctly completed. 
Notice that we instantiated $\ValidRun$ with $x=con$, $y_1=inc^1$.

\item Similarly for decrement commands.

\item Suppose the 2CM says \textit{`if counter 1 is zero then goto $x$ else goto $y$'}. 
Controller sends the token along edge $TZ^1$ to the first process in the memory component. 
The formula part 
$(CON\_TZ^1_{con} \to Z^1\_TOK_{z^1})$ 
checks that if the next non-memory process with the token 
is in component `zero $1$' then the control has $action = then^1$ and $cur = x$.
% and if the next non-memory process with the token 
% is in component 'non-zero $1$' then control has $action = else^1$ and $cur = y$. 
Note that if the counter $c$ is not-zero 
then the path to the process in component `zero $c$' is blocked; 
and if the counter $c$ is zero 
then the path to the process in component `non-zero $c$' is blocked.
\end{itemize} 
Hence we can simulate the 2CM and so encode an $n$-partial run 
in some path $\pi$ of $P^G$ 
that satisfies $\ltlG\ValidRun$
with $x=con$, $y_i=ord^{-1}(i)$.
\qed
\end{proof}

\begin{lemma}[$P^G$ by 2CM]\label{piltl_ny_undec:l3}
If 1) a path $\pi$ of $P^G$ (where $G$ has $2n+9$ nodes) 
  satisfies $\ltlG\ValidRun$ 
  for some assignment of the index variables $x,y_i$ where 
  the process $x$ is in the controller component, 
  and 2) the initialization phase of the (controller) process $x$ succeeded,
  then $\pi$ encodes an $n$-partial run of the 2CM.
\end{lemma}
\begin{proof}[idea]
Since the initialization phase is completed, 
then the process $x=con$ by Lemma~\ref{piltl_nc_undec:init_lemma}.
According to the description of the process templates, 
after the initialization phase the process $con$ starts simulation of the 2CM.
$\ltlG\ValidRun$ is true, 
therefore during the simulation all the processes correctly guesses the commands 
and the results.
Hence $\pi$ encodes an $n$-partial run of the 2CM.
\qed
\end{proof}

% \begin{enumerate}
% \item [\textit{L1.}]
% For every $n$, an $n$-partial run of 2CM is encoded by some path $\pi$ in $P^G$ 
%   (where $G \in \pgraph$ and has $2n+9$ nodes), 
%   that satisfies 
%   $\ltlG\ValidRun$ 
%   for the following assignment of the index variables: 
%   $x = con$ and $y_i = ord^{-1}(i)$, that is, $y_1=inc^1, y_2=dec^1, y_3=z^1$, etc.
% 
% \item [\textit{L2.}]
% If a path $\pi$ of $P^G$ satisfies $\ltlG\ValidRun$ 
%   for some assignment of the index variables $x,y_i$ in which 
%   the process $x$ is in the controller component, 
%   and the initialization phase of the process $x$ succeeded,  
%   then $\pi$ encodes an $n$-partial run of the 2CM.
% \end{enumerate}

Finally, the theorem follows from the lemma:
% Now we can prove the correctness of the construction using the lemmas above.
% \begin{proposition}\label{prop:nc_ltl_correct}
% The problem of halting a given 2CM $M$ 
% can be reduced to the problem $\PMCP_\pgraph(\Psnd,\{F\})$,
% where $\pgraph$, $F$ are independent of $M$,
% and a process template $P$ (dependent on $M$) 
% is as described above.
% \note{why is PMCP mentioned?}
% \end{proposition}
% 
\begin{lemma}[2CM reduction]\label{lemma: nc_ltl_correct}
A given 2CM $M$ halts if and only if
the answer to the problem $\PMCP_\pgraph(\{P\},\{F\})$\note{why is PMCP mentioned?}
is `No',
where $\pgraph$, $F$ (independent of $M$) and $P$ (dependent on $M$) are as described before.
\end{lemma}
\begin{proof}
% The proof follows from the above two lemmas:
% \begin{itemize}
%   \item ``The answer to the $\PMCP$ problem is ``No'' $\Rightarrow$ the 2CM halts'':
%   
  Suppose the answer to the $\PMCP$ problem is ``No''. 
  Hence there is a topology $G \in \pgraph$ and path $\pi$ of $P^G$,
  such that $\pi$ satisfies $\ltlG\ValidRun$, 
  but falsifies $\ltlG \neg HALT_{x}$ for some assignment of the index variables 
  $x,y_1,\ldots,y_9$. 
  Only the controller component has an atomic proposition $HALT$,
  therefore the process at vertex $x$ is in the controller component.
  Lets show that $x=con$, that is, 
  it is the process at vertex $con$ that reached the state $HALT$.
  Indeed, the process in the controller component can reach the state $HALT$
  only if the initialization phase succeded, which is possible only  
  if the process is at vertex $con$, so $x=con$.
  From Lemma~\ref{piltl_ny_undec:l3} it follows that the path $\pi$ encodes an $n$-partial run of the 2CM.
%   Lets show that $y_i=ord^{-1}(i)$ ($y_1=inc^1, y_2=dec^1,\ldots$).
%   If for some $i$, $y_i \ne ord^{-1}(i)$, 
%   then after receiving the token the process $i$ will send it to the sink 
%   (due to the graph structure) and the controller will not reach $HALT$ state.
%   Hence, $y_i=ord^{-1}(i)$.
  We just showed that process at $con$ reaches the state $HALT$, so does 
  2CM. Hence, the 2CM halts.

%   \item ``The 2CM halts $\Rightarrow$ the answer to the $\PMCP$ problem is ``No'''':
  
  Suppose the 2CM halts. 
  Hence there is an $n$-partial run that reaches a halting state of 2CM.
  From Lemma~\ref{piltl_ny_undec:l1} it follows that there is a path $\pi$ in $P^G$ for some $G$
  that encodes the $n$-partial run. 
%   Note that ``encodes'' means that a state of a process at vertex $con$ 
%   encodes the state of a configuration of the 2CM.
%   2CM halts, hence there is a global state of $P^G$ with state of process at $con$ equal to $HALT$.
%   From \textit{L2} it follows that the path $\pi$ 
  and
  satisfies $\ltlG\ValidRun$
  with $x=con$. Since $\ltlG(\neg HALT_{con})$ is false so is the formula $F$. 
  Hence the answer to $\PMCP$ is ``No''. 
  \qed
% \end{itemize}
\end{proof}
% Finally, the Theorem~\ref{thm:NC} immediately follows 
% from the construction of the graph $\pgraph$, process template $P$, formula $F$, 
% Proposition~\ref{prop: nc_ltl_correct} 
% and the undecidability of a non-halting problem for a 2CM.
\end{proof}

\begin{theorem}\label{thm:NC-CTL}
There exist a parameterized topology $\pgraph$ such that the problem $\PMCP_{\pgraph}(\Psnd,\nineexistsCTLmX)$ 
is undecidable. %Indeed, a non-halting problem for 2CM can be reduced to it.
\end{theorem}
\begin{proof}
The proof idea is the same as in the Theorem~\ref{thm:DA}. 
The parameterized topology and the process template are also the same. 
The formula $F$ is
\[
\neg \exists{x} \exists{y_1} \cdots \exists{y_8} : \ctlE (\ValidRun \ltlU HALT_x)
\]
where as in the Theorem~\ref{thm:DA}
$\ValidRun=\bigwedge_W  (CON\_W_{x} \to W\_TOK_{y_{ord(W)}})$ 
and $HALT_x$ is an atomic proposition of the controller component which is true 
only in the state corresponding to the halting state of the 2CM.
The formula $F$ is satisfied by some $P^G$ if and only if
the 2CM halts.

% \begin{itemize}
%   \item 
  Suppose the formula $F$ is falsified by some path $\pi$ in $P^G$.
  Then, by definition of the operator $\ltlU$, for some assignment of $x,y_1,\cdots,y_8$: 
  $\exists{i}: \pi[i] \models HALT_x \text{ and } \forall{k < i}: \pi[k] \models \ValidRun$
  ($HALT_x$ can be reached only by the controller process 
  at vertex $con$ of the topology on the Fig.~\ref{fig:fig_piltl_cn_undec} 
  , and only if the initialization phase completes, 
  see Lemma~\ref{piltl_nc_undec:init_lemma}). 
  All the guesses of all the processes are correct before 
  the controller reaches the halting state, 
  therefore it encodes an $n$-partial path of the 2CM that reaches the halting state.

%   \item 
  Suppose the 2CM halts. Then there is an $n$-partial path of the 2CM 
  that reaches a halting state. According to the Lemma~\ref{piltl_ny_undec:l1}, 
  there is a $\pi$ path of some $P^G$ that encodes the $n$-partial run and 
  satisfies $\ltlG \ValidRun$ with $x=con$. 
  Therefore, the path $\pi$ also satisfies $\ValidRun \ltlU HALT_x$ 
  with $x=con,y_i=ord^{-1}$. Hence, the path $\pi$ falsifies the formula $F$.
% \end{itemize}
\qed
\end{proof}

\begin{reptheorem}{thm:DA}
There exists a parameterized topology $\pgraph$ such that the problem $\PMCP_{\pgraph}(\Prcv,\nineallLTLmX)$ is undecidable.
%Indeed, a non-halting problem for 2CM can be reduced to it.
\end{reptheorem}
\begin{proof}[idea]
\ak{I don't think we need the whole proof, 
so here is an intuition why it works.}
% 
\iffig
\begin{figure}
\centering
\subfigure[Edges used in the simulation of a 2CM (without initializing edges).]{%
\input{fig_piltl_cn_undec}
\label{fig:fig_piltl_cn_undec_sim}}
% 
\quad
% 
\subfigure[Special edges are used only in the initialization phase.]{%
\input{fig_piltl_cn_undec_init}
\label{fig:fig_piltl_cn_undec_init}}
% 
\caption{Structure of the topology of processes, 
used in the proof of undecidability of 
$\PMCP$ of $\Prcv$ on general topologies wrt. $\nineallLTLmX$
($c\in\{1,2\}$).}
\label{fig:fig_piltl_cn_undec}
\end{figure}



% 
% \begin{figure}
%  \begin{subfigure}[b]{0.49\textwidth}
%     \centering
% %     \resizebox{\linewidth}{!}{
%       \input{fig_piltl_cn_undec}
% %     }  
%     \caption{Edges used in the simulation of a 2CM (without initializing edges).}
%     \label{fig:fig_piltl_cn_undec_sim}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.49\textwidth}
%     \centering
% %     \resizebox{\linewidth}{!}{
%       \input{fig_piltl_cn_undec_init}
% %     }
%     \caption{Special edges are used only in the initialization phase.}
%     \label{fig:fig_piltl_cn_undec_init}
%  \end{subfigure}
% %  
% \caption{Structure of the topology of processes, 
% used in the proof of undecidability of 
% $\PMCP$ of $\Prcv$ on general topologies wrt. $\nineallLTLmX$
% ($c\in\{1,2\}$).}
% \label{fig:fig_piltl_cn_undec}
% % 
% \end{figure}
\fi
\ak{label edges on Fig.(b)}
Similarly to the undecidability case of $\Psnd$, 
we can build 
a topology (Fig.~\ref{fig:fig_piltl_cn_undec}),
a process template $P$, 
a formula $F$, 
and then reduce the non-halting problem for a 2CM to $\PMCP$.

The process template has several components: 
`controller', `increment $c$', `decrement $c$', `zero $c$', `non-zero $c$', `memory of counter $c$'.
 
Consider a `memory of counter $c$' component:
\begin{itemize}
  \item 
  if the memory process has its $b=1$ then 
  it can receive the token only 
  via edges $NZ^c$ (release the token), 
          $DEC^c$ (set $b=0$ and release the token);
  
  \item 
  if the memory process has $b=0$ -- only via $Z^c$ (release the token), 
  $INC^c$ (set $b=1$ and release the token).
\end{itemize}
 
Components `increment $c$', `decrement $c$', `zero $c$', `non-zero $c$'
just passes the token further. 

Component `controller' has two phases: 
an initialization phase that ensures that the process is at vertex $con$, 
and a simulation of the 2CM phase. 

Consider `test counter $c$ for zero' command of the 2CM.
The controller guesses the result. If it guessed `zero', 
then it passes the token to process at $z^c$ (this is ensured in the formula),
and waits for the token from $Z^c$ direction. If the guess was wrong then one of the processes 
has $b=1$ and therefore cannot receive the token from $Z^c$ direction. So the command finished 
if and only if the token goes through all of the memory nodes.

Consider `increment $c$' command. The controller sends the token to process at $inc^c$ 
(ensured by the formula), and waits for the token from $M^c$ or $Z^c$ direction. 
The process $inc^c$ sends non-deterministically the token 
to the memory process with $b=0$ (the only possibility),
then the memory process releases the token. The token returns back to the controller
only if exactly one of the processes incremented its bit.

Similarly operate the simulation of other commands.

The formula is of a similar form as in the Theorem~\ref{thm:NC}:
\[
\forall x \forall y_1 \cdots \forall y_8: \,  \ltlG\ValidRun \to \ltlG\neg HALT_x
\]
where 
$\ValidRun = \bigwedge_W  (CON\_W_{x} \to W\_TOK_{y_{ord(W)}})$
.
\qed
\end{proof}

\todo{give full proof of CCbirings?}
\begin{reptheorem}{thm:DA}
The problem $\PMCP_{\textbf{BR}}(\Prcvsnd, \oneallLTLmX)$ is undecidable.
\end{reptheorem}
\begin{proof}[sketch]
The proof is inspired by the proof of an undecidability
of PMCP of uni-directional multi-valued token rings wrt. $\oneallLTLmX$~\cite{EN95},
which shows how $n$ steps of a 2CM can be simulated in a token ring of size $n$.

The process which has the token initially simulates 
the controller of the 2CM, 
and all other processes (call them memory processes) 
each store one bit for each of the two counters of the 2CM.

Assume that a subset of integer numbers represent commands of the 2CM, 
say 
0 $\mapsto$ `increment counter 1', 
1 $\mapsto$ `decrement counter 1',
2 $\mapsto$ `test for zero counter 1',
3 $\mapsto$ `increment counter 2', 
4 $\mapsto$ `decrement counter 2',
5 $\mapsto$ `test for zero counter 2'.
Every process has a command variable that represents the command to
be executed when it receives the token from direction {\sf ccw}.

If the controller sends the token in direction {\sf cw}, the memory
processes will increment (mod $6$) the command variable, allowing the
controller to encode which command should be executed. Every process
just continues to pass the token in direction {\sf cw}, until it
reaches the controller again.

If the controller sends the token in direction {\sf ccw}, then the 
memory processes try to execute the command currently
stored. If a memory process cannot execute the command 
(for instance, it is an `increment' and the process bit is already set to $1$, 
or it is a `test for zero' and the process bit is set to $0$), 
then it passes the token along direction {\sf ccw} and remembers that a
command is being tried. If the token reaches a memory process which can
execute the command 
(for a `test for zero' -- the process bit is set to $1$), 
then it does so and passes the token back in
direction {\sf cw}. The processes that remembered that a command is
being tried will receive the token from direction {\sf cw}, and know
that the command has been successfully executed. Similarly, if the
controller gets the token from {\sf cw}, he knows the command was
successful 
(for a `test for zero' it means the counter is not zero). 
If he gets it from {\sf ccw}, 
he knows that the command failed if it was an `increment', 
or that a `test for zero' returned ``yes, the counter is zero''.\sr{i think the proof should treat increment/decrement separate from test for zero}

If an `increment' command failed, 
the controller enters a loop in which it just passes the token in direction {\sf cw}.
After each `test for zero' command that returned ``yes, the counter is zero'', 
the controller sends the token in direction {\sf ccw} 
so that the memory processes know that the command was successfull.\sr{should probably point out that if test for zero failed then all processes have their pointer at the same command.}

In a state of the controller corresponding to a halting state of the 2CM, 
the atomic proposition $HALT$ holds (and only in that state).
Hence the formula to model check is of the form $\forall{i} \ltlG\neg HALT_i$.
% 
% The state of a memory process is represented by tuple $(b_1, b_2, cmd, stat)$, 
% where $b_1,b_2$ from $\{0,1\}$ represent the value of one bit 
% of the counter of the 2CM, the total number of bits $b_c$ set to $1$ 
% being equal to the value of counter $c$ ($c \in {1,2}$).
% The $cmd \in [6]$ and means the current command being executed by the controller:
% 1 $\mapsto$ `increment counter 1', 
% 2 $\mapsto$ `decrement counter 1',
% 3 $\mapsto$ `test for zero counter 1',
% 4 $\mapsto$ `increment counter 2', 
% 5 $\mapsto$ `decrement counter 2',
% 6 $\mapsto$ `test for zero counter 2'.
 \qed
\end{proof}

\todo{remove these for now?}

\blackout{
\begin{conjecture}
$\PMCP_{\textbf{Gr}}(\Prcvsnd, \piLTLmX)$ is undecidable. 
In particular, the non-halting problem for 2CM can be reduced to it.
\end{conjecture}\ak{leave this as is?}

\begin{proposition}
$\PMCP_{\pgraph}(\Psnd, \oneLTLmX)$ is decidable.
\end{proposition}
\begin{proof}
\todo{Write proof of dec of 1-LTL for N/Y}
The result above should hold for systems with global fairness, as in
~\cite{CTTV04}. The same decomposition should work, i.e., there is just one
hub which will eventually send back the token, and no other
communication is possible, nor can it be encoded into the spec.

If we use the fairness condition of~\cite{EN95}, we need to
distinguish hubs that can keep the token forever from hubs that
don't. Finally, if we use our own ``fairness'' condition, it is
unclear what happens (or is it the same as for~\cite{EN95} condition?).
\end{proof}
}

